Ultraviolet Positioning via TDOA: Error Analysis and System Prototype

This work performs the design, real-time hardware realization, and experimental evaluation of a positioning system by ultra-violet (UV) communication under photon-level signal detection. The positioning is based on time-difference of arrival (TDOA) principle. Time division-based transmission of synchronization sequence from three transmitters with known positions is applied. We investigate the positioning error via decomposing it into two parts, the transmitter-side timing error and the receiver-side synchronization error. The theoretical average error matches well with the simulation results, which indicates that theoretical fitting can provide reliable guidance and prediction for hardware experiments. We also conduct real-time hardware realization of the TDOA-based positioning system using Field Programmable Gate Array (FPGA), which is experimentally evaluated via outdoor experiments. Experimental results match well with the theoretical and simulation results.

==> Abstract.tex <==

\begin{abstract}
	
This work performs the design, real-time hardware realization, and experimental evaluation of a positioning system by ultra-violet (UV) communication under photon-level signal detection. The positioning is based on time-difference of arrival (TDOA) principle. Time division-based transmission of synchronization sequence from three transmitters with known positions is applied. We investigate the positioning error via decomposing it into two parts, the transmitter-side timing error and the receiver-side synchronization error. The theoretical average error matches well with the simulation results, which indicates that theoretical fitting can provide reliable guidance and prediction for hardware experiments. We also conduct real-time hardware realization of the TDOA-based positioning system using Field Programmable Gate Array (FPGA), which is experimentally evaluated via outdoor experiments. Experimental results match well with the theoretical and simulation results.


\end{abstract}

\begin{IEEEkeywords}
	Ultraviolet (UV) communication, positioning, TDOA, synchronization.
\end{IEEEkeywords}

==> Appendices.tex <==


\begin{appendices} 
%	\section{ Proof of Theorem \ref{theorem.meanvarforCase1} }  \label{appendix.meanvarforCase1}
%%	Combining Equation \eqref{equ.correlation for case 1}, we have the proof as follows.
%According to Eq. \eqref{equ.correlation for case 1} and Eq. \eqref{pnum1}, we have the following derivation.
%%Note that
%%	\begin{equation} 
%%		\operatorname{C}_{0,0}  \sim \sum_{i=1}^{L}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\},
%%	\end{equation}
%%where
%%	\begin{equation}
%%		n_{i} \sim \left[\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right)+\operatorname{Poi}\left((1-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\right].
%%	\end{equation} 
%\subsection{The expectation of $ \operatorname{C}_{0,0}  $}
%\subsubsection{The case where $ s_i$ lies in RANDOM part} 
%\begin{itemize}
%\item[*] If its two neighbors also lies in RANDOM part, we have $ {\bold E}\left(s_{i-1}s_{i}\right) = \frac{1}{4}$ and thus
%	\begin{equation}
%		\begin{aligned}
%		\mathrm{E_{1}}& \triangleq	{\bold E} \left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} \\ 
%			&={\bold E}\left\{{\bold E}\left[\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right) \mid \bm{s}\right]\right\} 
%			=0,
%		\end{aligned}
%	\end{equation}
%    \begin{equation}
%    	\begin{aligned}
%    	\mathrm{E_{2}}& \triangleq	{\bold E}\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%    	&	={\bold E}\left\{{\bold E}\left[\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\mid \bm{s}\right]\right\} 
%    		=(1-\varepsilon) \frac{\lambda_{s}}{2}.
%    	\end{aligned}
%    \end{equation}
%%	\begin{align} 
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  &=0,\\
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=(1-\varepsilon) \frac{\lambda_{s}}{2},
%%	\end{align}
%\item[*] If $ s_{i-1}=0$ when the boundary is between  $ s_{i-1}$ and  $ s_{i}$ or $ i=1 $, we have $	\mathrm{E_{1}}=0$, $\mathrm{E_{2}}=(1-\varepsilon) \frac{\lambda_{s}}{2}$.
%%\begin{equation}
%%	\begin{aligned}
%%%		{\bold E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  
%%%		=\varepsilon\mathrm{E}\left\{2\lambda_{s} s_{i-1}s_{i}-\lambda_{s} s_{i-1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%		\mathrm{E_{1}}=0,~~~\mathrm{E_{2}}=(1-\varepsilon) \frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		{\bold E}\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%		&=\left(1-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}\\
%%		=(1-\varepsilon) \frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%\end{itemize}
%\subsubsection{The case where $ s_i $ lies in $1-0$ alternate part} 
%\begin{itemize}
%\item[*] If its two neighbors also lie in $1-0$ alternate part, we have ${\bold E}(s_{i-1}s_i) = 0$. For $ (\alpha L - 2) $ items which don't lie in boundaries, we have $ {\bold E}\left(s_{i}\right) =\frac{1}{2}$ and $ {\bold E}\left(s_{i-1}\right) =\frac{1}{2}$, and $\mathrm{E_{1}}=(-\varepsilon) \frac{\lambda_{s}}{2}$, $\mathrm{E_{2}}=(1-\varepsilon) \frac{\lambda_{s}}{2}$.
%%	\begin{equation}
%%		\begin{aligned}
%%%			{\bold E}&\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  
%%%			=\mathrm{E}\left\{\mathrm{E}\left[\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right) \mid \bm{s}\right]\right\} \\
%%%			&=\varepsilon\mathrm{E}\left\{2\lambda_{s} s_{i-1}s_{i}-\lambda_{s} s_{i-1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%			\mathrm{E_{1}}=(-\varepsilon) \frac{\lambda_{s}}{2},~~~\mathrm{E_{2}}=(1-\varepsilon) \frac{\lambda_{s}}{2}.
%%		\end{aligned}
%%	\end{equation}
%%	\begin{equation}
%%		\begin{aligned}
%%			{\bold E}&\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%			=\mathrm{E}\left\{\mathrm{E}\left[\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\mid \bm{s}\right]\right\} \\
%%%			&=\left(1-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%			=(1-\varepsilon) \frac{\lambda_{s}}{2}.
%%		\end{aligned}
%%	\end{equation}
%\item[*] If $ s_{i-1}$ lies in RANDOM part and $ s_i=1 $ when the boundary is between  $ s_{i-1}$ and $ s_{i}$, we have $\mathrm{E_{1}}	=\varepsilon( \frac{\lambda_{s}}{2}+\lambda_{b})$, $\mathrm{E_{2}}=(1-\varepsilon) \left(\lambda_{s}+\lambda_{b}\right)$.
%%	\begin{equation}
%%	\begin{aligned}
%%%		{\bold E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%%		&=\varepsilon\mathrm{E}\left\{2\lambda_{s} s_{i-1}s_{i}-\lambda_{s} s_{i-1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}\\
%%	\mathrm{E_{1}}	=\varepsilon( \frac{\lambda_{s}}{2}+\lambda_{b}),~~~\mathrm{E_{2}}=(1-\varepsilon) \left(\lambda_{s}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		{\bold E}\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%		&=\left(1-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}\\
%%		=(1-\varepsilon) \left(\lambda_{s}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%%	\begin{align} 
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  &=(-\varepsilon) \frac{\lambda_{s}}{2},\\
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=(1-\varepsilon) \frac{\lambda_{s}}{2}, 
%%	\end{align}
%\item[*] If $ s_i=0 $ lies at the end of $1-0$ alternate part with $ s_{i-1}=1 $, we have $\mathrm{E_{1}}	=-\varepsilon( \lambda_{s}+\lambda_{b})$, $\mathrm{E_{2}}=-(1-\varepsilon) \lambda_{b}$.
%%	\begin{equation}
%%	\begin{aligned}
%%%		{\bold E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  
%%%		&=\varepsilon\mathrm{E}\left\{2\lambda_{s} s_{i-1}s_{i}-\lambda_{s} s_{i-1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}\\
%%	\mathrm{E_{1}}	=-\varepsilon( \lambda_{s}+\lambda_{b}),~~~\mathrm{E_{2}}		=-(1-\varepsilon) \lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		{\bold E}\left\{\operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%		&=\left(1-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}\\
%%		=-(1-\varepsilon) \lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%\end{itemize}
%By adding up components above, the expectation of $ \operatorname{C}_{0,0}  $ is given by
%	\begin{equation}
%		\begin{aligned}
%			{\bold E}\left(\operatorname{C}_{0,0}\right)
%%			=&L(1-\alpha)\left[0+(1-\varepsilon) \frac{\lambda_{s}}{2}\right]
%%			+(\alpha L -2)\left[(-\varepsilon) \frac{\lambda_{s}}{2}+(1-\varepsilon) \frac{\lambda_{s}}{2}\right]\\
%%			&+\left[\varepsilon( \frac{\lambda_{s}}{2}+\lambda_{b})+(1-\varepsilon) \left(\lambda_{s}+\lambda_{b}\right)\right]
%%			+\left[-\varepsilon( \lambda_{s}+\lambda_{b})-(1-\varepsilon) \lambda_{b}\right]\\
%			=L \frac{\lambda_{s}}{2}[1-(1+\alpha) \varepsilon]+\varepsilon \frac{\lambda_{s}}{2}.
%		\end{aligned}
%	\end{equation}
%%	\begin{align} 
%%		\mathrm{E}\left(\operatorname{C}_{0,0}\right)=L \frac{\lambda_{s}}{2}[1-(1+\alpha) \varepsilon] 
%%		%\label{mean for case1.equation}
%%	\end{align}
%\subsection{The expectation of $ \operatorname {\bold V a r }\left(\operatorname{C}_{0,0} \right) $}
%Since two parts $ \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) $ and from $ \operatorname{Poi}\left(\left(1-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) $ are statistically independent, for both cases where $s_i$ lies in the random part or $1-0$ alternate part, we have
%\begin{equation}
%	\begin{aligned}
%		&{\bold E}\left\{\operatorname {\bold V a r } \left(\operatorname{Poi}\left((1-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\times\left(2 s_{i}-1\right)\right)\right\}\\
%		&={\bold E}\left\{{\bold E}\left[\operatorname {\bold V a r } \left(\operatorname{Poi}\left((1-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\times\left(2 s_{i}-1\right)\right)\mid \bm{s}\right]\right\}
%%		&={\bold E}\left\{{\bold E}\left[ (1-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\times\left(2 s_{i}-1\right)^2\mid \bm{s}\right]\right\}
%%		={\bold E}\left\{(1-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right\}
%		=(1-\varepsilon)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right), \\
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		&{\bold E}\left\{\operatorname{\bold Var}\left(\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right)\right\}
%%		&={\bold E}\left\{{\bold E}\left[\operatorname {\bold V a r } \left(\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right)\times\left(2 s_{i}-1\right)\right)\mid \bm{s}\right]\right\}
%%		&={\bold E}\left\{{\bold E}\left[ \varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\times\left(2 s_{i}-1\right)^2\mid \bm{s}\right]\right\}
%%		={\bold E}\left\{\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right\}
%		=\varepsilon\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%	\end{aligned}
%\end{equation}
%%\begin{align}
%%	\mathrm{E}\left\{\operatorname { V a r } \left(\operatorname{Poi}\left((1-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\times\left(2 s_{i}-1\right)\right)\right\}&=(1-\varepsilon)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right) \\
%%	\mathrm{E}\left\{\operatorname{Var}\left(\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right)\right\}&=\varepsilon\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)
%%\end{align}
%Thus, the expectation of variance of $ \operatorname{C}_{0,0}  $ is given by 
%\begin{align}
%	{\bold E}\left(\operatorname{\bold Var}\left(\operatorname{C}_{0,0}\right)\right)=L\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)\left(1-\varepsilon+\varepsilon\right)=L\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%\end{align}
%In subsequent proofs, some of the detailed formula derivation steps are simplified due to the similarity with the proof of Theorem \ref{theorem.meanvarforCase1}.
%\section{ Proof of Theorem \ref{theorem.meanvarforCase2} }  \label{appendix.meanvarforCase2}
%According to Eq. \eqref{equ.correlation for case 2} and Eq. \eqref{pnum2}, we have the following derivation.
%%Note that
%%\begin{equation}
%%	\operatorname{C}_{0,k}  \sim \sum_{i=1}^{L}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\},
%%\end{equation}	
%%where
%%\begin{equation}
%%	\begin{aligned}
%%	n_{i} \sim \left[\operatorname{Poi}\left((1-\frac{k}{n})\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)
%%	+\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)
%%    +\operatorname{Poi}\left((\frac{k}{n}-\varepsilon)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right)\right].
%%	\end{aligned}
%%\end{equation} 
%\subsection{The expectation of $ \operatorname{C}_{0,k}  $}
%Let
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{3}} \triangleq {\bold E} \left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} ,
%		%		&=(1-\frac{k}{n})\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{4}} \triangleq {\bold E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} ,
%		%	=\varepsilon\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{5}}\triangleq {\bold E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} .
%		%     &=\left(\frac{k}{n}-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+1}-\lambda_{s}s_{i+1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%	\end{aligned}
%\end{equation}
%%First, when $ s_i$ with its two neighbors are in RANDOM part, $ \mathrm{E}\left(s_{i+1}s_{i}\right) = \frac{1}{4}$.
%%$ \bm{B.1} $ Firstly, considering the case where $ s_i$ lies in RANDOM part,
%\subsubsection{The case where $ s_i$ lies in RANDOM part} 
%\begin{itemize}
%\item [*] If its two neighbors also lie in RANDOM part, we have $ {\bold E}\left(s_{i-1}s_{i}\right) = \frac{1}{4}$ and thus $\mathrm{E_{3}}=(1-\frac{k}{n}) \frac{\lambda_{s}}{2}$, $\mathrm{E_{4}}=\varepsilon \frac{\lambda_{s}}{2}$, $\mathrm{E_{5}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%		&=(1-\frac{k}{n})\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%		\mathrm{E_{3}}=(1-\frac{k}{n}) \frac{\lambda_{s}}{2},
%%		~~~\mathrm{E_{4}}=\varepsilon \frac{\lambda_{s}}{2},
%%		~~~\mathrm{E_{5}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%	=\varepsilon\mathrm{E}\left\{2\lambda_{s}s_{i}^2-\lambda_{s}s_{i}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%		=\varepsilon \frac{\lambda_{s}}{2},
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%%     &=\left(\frac{k}{n}-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+1}-\lambda_{s}s_{i+1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%		=0.
%%	\end{aligned}
%%\end{equation}
%\item [*] If $ s_{i+1}=1$ when the boundary is between  $ s_{i}$ and  $ s_{i+1}$ or $ s_{i+1}=0$ when $ i=L $, we have $\mathrm{E_{3}} =(1-\frac{k}{n}) \frac{\lambda_{s}}{2}$, $\mathrm{E_{4}}=\varepsilon \frac{\lambda_{s}}{2}$, $\mathrm{E_{5}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		\mathrm{E_{3}} =(1-\frac{k}{n}) \frac{\lambda_{s}}{2},
%%		~~~\mathrm{E_{4}}=\varepsilon \frac{\lambda_{s}}{2},
%%		~~~\mathrm{E_{5}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=\varepsilon \frac{\lambda_{s}}{2},
%%	\end{aligned}
%%\end{equation}
%%For both cases of $ s_{i+1} =0 $ and $ s_{i+1}=1 $, we have
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=0.
%%\mathrm{E_{5}}=0.
%%	\end{aligned}
%%\end{equation}
%\end{itemize}
%%\begin{align} 
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=(1-\frac{k}{n}) \frac{\lambda_{s}}{2},\\
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  &=\varepsilon \frac{\lambda_{s}}{2},\\
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=0,
%%\end{align}
%%When $ s_i $ with its two neighbors are in $\{1,0,...\} $ part, $ \mathrm{E}\left(s_{i+1}s_{i}\right) = 0$.
%%$ \bm{B.2} $ Considering the scenario where $ s_i $ lies in $1-0$ alternate part, 
%\subsubsection{The case where $ s_i $ lies in $1-0$ alternate part}
%\begin{itemize}
%\item [*] If its two neighbors also lie in $1-0$ alternate part, we have $ {\bold E}\left(s_{i+1}s_{i}\right) = 0$. For $ (\alpha L - 2) $ items which don't lie in boundaries, we have $ {\bold E}\left(s_{i}\right) =\frac{1}{2}$ and $ {\bold E}\left(s_{i+1}\right) =\frac{1}{2}$. And $\mathrm{E_{3}}=(1-\frac{k}{n}) \frac{\lambda_{s}}{2}$, $\mathrm{E_{4}}=\varepsilon \frac{\lambda_{s}}{2}$, $\mathrm{E_{5}}=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2}$.
%%\begin{align} 
%%%	&\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} =(1-\frac{k}{n}) \frac{\lambda_{s}}{2},\\
%%\mathrm{E_{3}}=(1-\frac{k}{n}) \frac{\lambda_{s}}{2},
%%~~~\mathrm{E_{4}}=\varepsilon \frac{\lambda_{s}}{2},
%%~~~\mathrm{E_{5}}=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2}.
%%%	&\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=\varepsilon \frac{\lambda_{s}}{2},
%%%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2},
%%\end{align}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%\item [*] If $ s_{i+1}$ lies in RANDOM part and $ s_i=0 $ when the boundary is between $ s_{i}$ and $ s_{i+1}$, we have $\mathrm{E_{3}}=(1-\frac{k}{n}) \left(-\lambda_{b}\right)$, $\mathrm{E_{4}}=\varepsilon \left(-\lambda_{b}\right)$, $\mathrm{E_{5}}=-(\frac{k}{n}-\varepsilon)(\frac{\lambda_{s}}{2}+\lambda_{b})$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		\mathrm{E_{3}}=(1-\frac{k}{n}) \left(-\lambda_{b}\right),
%%		~~~\mathrm{E_{4}}=\varepsilon \left(-\lambda_{b}\right),
%%		~~~\mathrm{E_{5}}=-(\frac{k}{n}-\varepsilon)(\frac{\lambda_{s}}{2}+\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=\varepsilon \left(-\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%\begin{align} 
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=(1-\frac{k}{n}) \frac{\lambda_{s}}{2},\\
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  &=\varepsilon \frac{\lambda_{s}}{2},
%%	%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2},
%%\end{align}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} =-(\frac{k}{n}-\varepsilon)(\frac{\lambda_{s}}{2}+\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%\item [*] If $ s_i=1 $ lies at the start of $1-0$ alternate part with $ s_{i+1}=0 $, we have $\mathrm{E_{3}}=(1-\frac{k}{n}) \left(\lambda_{s}+\lambda_{b}\right)$, $\mathrm{E_{4}}=\varepsilon \left(\lambda_{s}+\lambda_{b}\right)$, $\mathrm{E_{5}}=(\frac{k}{n}-\varepsilon)(\lambda_{b})$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%		\mathrm{E_{3}}=(1-\frac{k}{n}) \left(\lambda_{s}+\lambda_{b}\right),
%%		~~~\mathrm{E_{4}}=\varepsilon \left(\lambda_{s}+\lambda_{b}\right),
%%		~~~\mathrm{E_{5}}=(\frac{k}{n}-\varepsilon)(\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=\varepsilon \left(\lambda_{s}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		=(\frac{k}{n}-\varepsilon)(\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%\end{itemize}
%Based on the above results, the expectation of $ \operatorname{C}_{0,k}  $ is given by
%\begin{align} 
%	{\bold E}\left(\operatorname{C}_{0,k}\right)=L \frac{\lambda_{s}}{2}[1-(1+\alpha) (\frac{k}{n}-\varepsilon)]+(\frac{k}{n}-\varepsilon)\frac{\lambda_{s}}{2}.
%	%\label{mean for case2.equation}
%\end{align}
%\subsection{The expectation of $ \operatorname {\bold V a r }\left(\operatorname{C}_{0,k} \right) $}
%Similar to that of Case 1, the expectation of variance of $ \operatorname{C}_{0,k}  $ is given by
%\begin{align}
%	{\bold E}\left(\operatorname{\bold Var}\left(\operatorname{C}_{0,k}\right)\right)=L\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%\end{align}
%\section{ Proof of Theorem \ref{theorem.covforCase2} }  \label{appendix.covforCase2}
%According to Eq. \eqref{pre_pnum3} and Eq. \eqref{pnum3}, we have the following derivation.
%%Note that
%%\begin{equation} 
%%	\operatorname{C}_{0,0}  \sim \sum_{i=1}^{L}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\},
%%\end{equation}
%%where
%%\begin{equation}
%%	\begin{aligned}
%%	n_{i} \sim \left[\operatorname{Poi}\left((\frac{k}{n}-\varepsilon)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)
%%	+\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right)
%%	+\operatorname{Poi}\left((1-\frac{k}{n})\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\right].
%%	\end{aligned}
%%\end{equation} 
%
%By analysis, the covariance is mainly composed of covariance of Poisson random variables, such as $ \operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\} $ for $ i-1=j $, which means $\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right)$ and $ \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right) $ are actually the same random variable as a result that they are from Poisson process during the same period of time.
%\begin{equation}
%	\begin{aligned}
%		&\mathrm{E_{6}}\triangleq\\
%		&{\bold E}\left(\operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right),
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		&\mathrm{E_{7}} \triangleq {\bold E}\left(\operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right),\\
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		&\mathrm{E_{8}}\triangleq\\
%		&{\bold E}\left(\operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right).\\
%	\end{aligned}
%\end{equation}
%%First, when $ s_i$ with its two neighbors are in RANDOM part, $ \mathrm{E}\left(s_{i-1}s_{i}\right) = \frac{1}{4}$.\\
%\subsection{The case where $ s_j$ lies in RANDOM part} 
%%Firstly, consider the case where $ s_j$ lies in RANDOM part. \\
%For $ \left(1-\alpha\right)L $ pairs of $ \left(i,j\right) $ with $ i=j $, we have
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{6}}
%		={\bold E}\left\{\left(2 s_{j}-1\right)\left(2 s_{j}-1\right)\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}
%		=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%	\end{aligned}
%\end{equation}
%\subsubsection{The case that two neighbors of $ s_j $ also lie in RANDOM part} We have ${\bold E}\left(s_{j}s_{j+1}\right) = \frac{1}{4}$.
%For $ \left[\left(1-\alpha\right)L-2\right] $ pairs of $ \left(i,j\right) $ with $ i-1=j $, we have $\mathrm{E_{7}} =0$, $\mathrm{E_{8}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%	     \left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\\
%%\mathrm{E_{7}} 
%%		={\bold E}\left\{\left(2 s_{j+1}-1\right)\left(2 s_{j}-1\right)\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}
%%		=0,~~~\mathrm{E_{8}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		\mathrm{E_{8}}={\bold E}\left\{\left(2 s_{j+1}-1\right)\left(2 s_{j}-1\right)\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}
%%		=0.\\
%%	\end{aligned}
%%\end{equation}
%%For $ \left(1-\alpha\right)L $ pairs of $ \left(i,j\right) $ with $ i-1=j $, 
%%\begin{align}
%%	&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)=0,\\
%%	&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\end{align}
%\subsubsection{The case that $ s_{j+1}=1$ when the boundary is between $ s_{j}$ and $ s_{j+1}$ or $ s_{j+1}=0 $ when $ j=L $}
%For $ 2 $ pairs of $ \left(i,j\right) $ with $ i-1=j $, we have $\mathrm{E_{7}}=0$, $\mathrm{E_{8}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)
%%		\mathrm{E_{7}}=0,~~~\mathrm{E_{8}}=0.\\
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%%	     \left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=0.\\
%%	\end{aligned}
%%\end{equation}
%%For $ \left(1-\alpha\right)L $ pairs of $ \left(i,j\right) $ with $ i=j $,
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=\mathrm{E}\left\{\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\mid \bm{s} \right\}  \\
%%		&=\mathrm{E}\left\{\left(2 s_{i}-1\right)\left(2 s_{i}-1\right)\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\right\}\\
%%		&=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%When $ s_i $ with its two neighbors are in $\{1,0,...\} $ part, $ \mathrm{E}\left(s_{i-1}s_{i}\right) = 0$.\\
%\subsection{The case where $ s_j$ lies in $1-0$ alternate part} 
%For $ \alpha L $ pairs of $ \left(i,j\right) $ with $ i=j $, we have $\mathrm{E_{6}}=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%%%		  \left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\\
%%		\mathrm{E_{6}}=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that two neighbors of $ s_j $ also lie in $1-0$ alternate part} We have $ {\bold E}\left(s_{j}s_{j+1}\right) = 0$. There are $ (\alpha L-2) $ items not lying around boundaries with $ {\bold E}\left(s_{j}\right) =\frac{1}{2}$ and $ {\bold E}\left(s_{j+1}\right) =\frac{1}{2}$. For $ (\alpha L-2) $ pairs of $ \left(i,j\right) $ with $ i-1=j $, we have $\mathrm{E_{7}}=\left(- \varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)$, $\mathrm{E_{8}}= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%	     \left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)
%%		\mathrm{E_{7}}=\left(- \varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%		~~~\mathrm{E_{8}}= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		\mathrm{E_{3}}= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $ s_{j+1}$ lies in RANDOM part and $ s_j=0 $ when the boundary is between  $ s_{j}$ and $ s_{j+1}$} 
% For 1 pair of $ \left(i,j\right) $ with $ i-1=j $, we have $\mathrm{E_{7}}=0$, $\mathrm{E_{8}}= -\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2}$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{7}}=0,
%%~~~\mathrm{E_{8}}= -\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		\mathrm{E_{3}}= -\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $ s_j=1 $ as the start of $1-0$ alternate part with $ s_{j+1}=0 $} 
%For 1 pair of $ \left(i,j\right) $ with $ i-1=j $, we have $\mathrm{E_{7}}	=-\varepsilon \left(\lambda_{s}+\lambda_{b}\right)$, $\mathrm{E_{8}}= -\left(\frac{k}{n}-\varepsilon \right)\lambda_{b}$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)
%%	\mathrm{E_{7}}	=-\varepsilon \left(\lambda_{s}+\lambda_{b}\right),
%%	~~~\mathrm{E_{8}}= -\left(\frac{k}{n}-\varepsilon \right)\lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		\mathrm{E_{3}}= -\left(\frac{k}{n}-\varepsilon \right)\lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=\left(- \varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%For $ \alpha L $ pairs of $ \left(i,j\right) $ with $ i=j $,
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=\mathrm{E}\left\{\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\mid \bm{s} \right\}  \\
%%		&=\mathrm{E}\left\{\left(2 s_{i}-1\right)\left(2 s_{i}-1\right)\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right)\right\}\\
%%		&=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%
%By adding up components above, the mathematical expectation of covariance is,
%\begin{equation}
%\begin{aligned}
%	{\bold E}\left\{\operatorname{\bold Cov}\left(\operatorname{C}_{0,0}, \operatorname{C}_{0, k}\right)\right\}
%%	&=L\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)\left[1-(1+\alpha) \frac{k}{n}\right]+(\frac{k}{n}-\varepsilon)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)+\frac{k}{n} \frac{\lambda_{s}}{2}+\varepsilon \lambda_{b}\\
%	=L\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)\left[1-(1+\alpha) \frac{k}{n}\right]
%	+\frac{k}{n}\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)-\varepsilon \frac{\lambda_{s}}{2}.
%\end{aligned}
%\end{equation}
%\section{ Proof of Theorem \ref{theorem.meanvarforCase3} }  \label{appendix.meanvarforCase3}
%According to Eq. \eqref{equ.correlation for case 3} and Eq. \eqref{pnum4}, we have the following derivation.
%%Note that
%%\begin{equation} 
%%	\operatorname{C}_{2m,k}  \sim \sum_{i=1}^{L}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\},~~2m \leq \min\{\alpha L, \frac{1-\alpha}{2}L\},
%%\end{equation}	
%%where
%%\begin{equation}
%%	\begin{aligned}
%%	n_{i} \sim \left[\operatorname{Poi}\left((1-\frac{k}{n})\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right)
%%	+\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right)
%%	+\operatorname{Poi}\left((\frac{k}{n}-\varepsilon)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right)\right]
%%	\end{aligned}
%%\end{equation} 
%\subsection{The expectation of $ \operatorname{C}_{2m,k}  $}
%Let
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{9}}\triangleq{\bold E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} ,
%		%		&=(1-\frac{k}{n})\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+2m}-\lambda_{s}s_{i+2m}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{10}}\triangleq{\bold E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\},  
%		%		&=\varepsilon\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+2m}-\lambda_{s}s_{i+2m}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{11}}\triangleq{\bold E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} .
%		%		&=\left(\frac{k}{n}-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+2m+1}-\lambda_{s}s_{i+2m+1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%	\end{aligned}
%\end{equation}
%\subsubsection{The case where $ s_i$ lies in RANDOM part}
%\begin{itemize}
%	\item [*] When $1 \leq i \leq (L-2m-1) $, we have $ {\bold E}\left(s_{i}s_{i+2m}\right) = \frac{1}{4}$ and $ {\bold E}\left(s_{i}s_{i+2m+1}\right) = \frac{1}{4}$, since $ s_{j},s_{j+2m}$ and $s_{j+2m+1} $ lie in RANDOM part. There are $ \left(1-\alpha\right)L-2m-1 $ cumulative items in the $ \operatorname{C}_{2m,k} $ following ${\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0$ with $1 \leq i \leq (L-2m-1)$.
%%\begin{equation}
%%	{\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0, 1 \leq i \leq (L-2m-1).
%%\end{equation}
%%Let
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E_{7}}\triangleq{\bold E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} ,
%%		%		&=(1-\frac{k}{n})\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+2m}-\lambda_{s}s_{i+2m}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E_{8}}\triangleq{\bold E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\},  
%%		%		&=\varepsilon\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+2m}-\lambda_{s}s_{i+2m}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E_{9}}\triangleq{\bold E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} .
%%		%		&=\left(\frac{k}{n}-\varepsilon\right)\mathrm{E}\left\{2\lambda_{s}s_{i}s_{i+2m+1}-\lambda_{s}s_{i+2m+1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%	\end{aligned}
%%\end{equation}
%\item [*] When $ i=L-2m $, we have $ s_{i+2m} $ lying in RANDOM part as well as $ s_{i+2m+1} = 0$. There are $ 1 $ cumulative item in the $ \operatorname{C}_{2m,k} $ following
%\begin{equation}
%	\begin{aligned}
%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%        \mathrm{E_{9}}=(1-\frac{k}{n}){\bold E}\left\{2\lambda_{s}s_{i}s_{i+2m}-\lambda_{s}s_{i+2m}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%		=0,~~~\mathrm{E_{10}}=0,~~~\mathrm{E_{11}}=0.
%	\end{aligned}
%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  
%%\mathrm{E_{10}}=\varepsilon{\bold E}\left\{2\lambda_{s}s_{i}s_{i+2m}-\lambda_{s}s_{i+2m}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%		=0,
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} 
%%\mathrm{E_{11}}=\left(\frac{k}{n}-\varepsilon\right){\bold E}\left\{2\lambda_{s}s_{i}s_{i+2m+1}-\lambda_{s}s_{i+2m+1}+2\lambda_{b}s_{i}-\lambda_{b}\right\}
%%		=0.
%%	\end{aligned}
%%\end{equation}
%%Thus, 
%%\begin{equation}
%%	{\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0, i=L-2m.
%%\end{equation}
%\item [*] When $(L-2m+1) \leq i \leq L $, we have $ s_{i+2m} = 0$ as well as $ s_{i+2m+1} = 0$. There are $ 2m $ cumulative item in the $ \operatorname{C}_{2m,k} $ following $\mathrm{E_{9}}=0$, $\mathrm{E_{10}}=0$, $\mathrm{E_{11}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=0,
%%\mathrm{E_{9}}=0,
%%~~~\mathrm{E_{10}}=0,
%%~~~\mathrm{E_{11}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=0,
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=0.
%%	\end{aligned}
%%\end{equation}
%%Thus, 
%%\begin{equation}
%%	{\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0, (L-2m+1) \leq i \leq L.
%%\end{equation}
%\end{itemize}
%%If $ s_{i} $ lies in RANDOM part, there are $ \left(1-\alpha\right)L $ cumulative items in the $ \operatorname{C}_{2m,k} $ in total follows
%%\begin{equation}
%%	{\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0.
%%\end{equation}
%\subsubsection{The case where $ s_i$ lies in $1-0$ alternate part}
%\begin{itemize}
%	\item [*] When $ \left(\frac{1-\alpha}{2} L +2\right) \leq i \leq \left(\frac{1+\alpha}{2}L-2m-1\right) $, we have $ {\bold E}\left(s_{i}s_{i+2m}\right) = 1$ and $ {\bold E}\left(s_{i}s_{i+2m+1}\right) = 0$. There are $ \alpha L-2m-2 $ cumulative items in the $ \operatorname{C}_{2m,k} $ following $\mathrm{E_{9}}=(1-\frac{k}{n}) \frac{\lambda_{s}}{2}$, $\mathrm{E_{10}}=\varepsilon \frac{\lambda_{s}}{2}$, $\mathrm{E_{11}}=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2}$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		\mathrm{E_{9}}=(1-\frac{k}{n}) \frac{\lambda_{s}}{2},
%%		~~~\mathrm{E_{10}}=\varepsilon \frac{\lambda_{s}}{2},
%%		~~~\mathrm{E_{11}}=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=\varepsilon \frac{\lambda_{s}}{2},
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%\item [*] When $  i = \left(\frac{1+\alpha}{2} L-2m\right) $, we have $ s_{i}=s_{i+2m}=0$ and ${\bold E}\left(s_{i}s_{i+2m+1}\right) = 0$. $ s_{i+2m} $ is the end of $1-0$ alternate part. There are $ 1 $ cumulative item in the $ \operatorname{C}_{2m,k} $ following $\mathrm{E_{9}}=-(1-\frac{k}{n}) \lambda_{b}$, $\mathrm{E_{10}}=-\varepsilon \lambda_{b}$, $\mathrm{E_{11}}=-\left(\frac{k}{n}-\varepsilon\right)(\frac{\lambda_{s}}{2}+\lambda_{b})$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		\mathrm{E_{9}}=-(1-\frac{k}{n}) \lambda_{b},
%%		~~~	\mathrm{E_{10}}=-\varepsilon \lambda_{b},
%%		~~~\mathrm{E_{11}}=-\left(\frac{k}{n}-\varepsilon\right)(\frac{\lambda_{s}}{2}+\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=-\varepsilon \lambda_{b},
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		=-\left(\frac{k}{n}-\varepsilon\right)(\frac{\lambda_{s}}{2}+\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%\item [*] When $  i = \left(\frac{1-\alpha}{2} L +1\right) $, we have $ s_{i}=s_{i+2m}=1$ and ${\bold E}\left(s_{i}s_{i+2m+1}\right) = 0$. $ s_{i} $ is the start of $1-0$ alternate part. There are $ 1 $ cumulative item in the $ \operatorname{C}_{2m,k} $ following $\mathrm{E_{9}}	=(1-\frac{k}{n}) (\lambda_{s}+\lambda_{b})$, $\mathrm{E_{10}}=\varepsilon (\lambda_{s}+\lambda_{b})$, $\mathrm{E_{11}}=\left(\frac{k}{n}-\varepsilon\right)\lambda_{b}$.
%%\begin{equation}
%%	\begin{aligned}
%%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%	\mathrm{E_{9}}	=(1-\frac{k}{n}) (\lambda_{s}+\lambda_{b}),
%%	~~~\mathrm{E_{10}}=\varepsilon (\lambda_{s}+\lambda_{b}),
%%	~~~\mathrm{E_{11}}=\left(\frac{k}{n}-\varepsilon\right)\lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}=\varepsilon (\lambda_{s}+\lambda_{b}),
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		\mathrm{E}&\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}
%%		=\left(\frac{k}{n}-\varepsilon\right)\lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%\item [*] When $ \left(\frac{1+\alpha}{2} L-2m+1 \leq i \leq \frac{1+\alpha}{2} L\right) $, we have $ {\bold E}\left(s_{i}s_{i+2m}\right) = \frac{1}{4}$ and $ {\bold E}\left(s_{i}s_{i+2m+1}\right) = \frac{1}{4}$. There are $ 2m $ cumulative items in the $ \operatorname{C}_{2m,k} $ following ${\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0$.
%%\begin{equation}
%%	{\bold E}\left\{n_{i} \times\left(2 s_{i}-1\right)\right\}=0.
%%\end{equation}
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=(1-\frac{k}{n}) \frac{\lambda_{s}}{2},\\
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i+2m}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\}  &=\varepsilon \frac{\lambda_{s}}{2},\\
%%	\mathrm{E}\left\{\operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i+2m+1}+\lambda_{b}\right)\right) \times\left(2 s_{i}-1\right)\right\} &=-(\frac{k}{n}-\varepsilon) \frac{\lambda_{s}}{2},
%%\end{align}
%\end{itemize}
%Thus, the expectation of  $ \operatorname{C}_{2m,k} $ is given by
%\begin{align}
%	{\bold E}&\left(\operatorname{C}_{2m, k}\right)
%	=\frac{\lambda_{s}}{2}\left\{(\alpha L-2 m)\left[1-2\left(\frac{k}{n}-\varepsilon\right)\right]+\left(\frac{k}{n}-\varepsilon\right)\right\},
%     2m \leq \min\{\alpha L, \frac{1-\alpha}{2}L\}.
%	%\label{mean for case3.equation}
%\end{align}
%\subsection{The expectation of $ \operatorname {\bold V a r }\left(\operatorname{C}_{2m,k} \right) $}
%Similar to  of Case 1, the expectation of variance of $ \operatorname{C}_{2m,k}  $ is given by
%\begin{align}
%	{\bold E}&\left(\operatorname{\bold Var}\left(\operatorname{C}_{2m,k}\right)\right)=\left(L-2m\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%	 2m \leq \min\{\alpha L, \frac{1-\alpha}{2}L\}.
%\end{align}
%Compared to Case 1, the cumulative terms from  missed $ 2m $ symbols in the variance calculation are ruled out.
%\section{ Proof of Theorem \ref{theorem.covforCase3} }  \label{appendix.covforCase3}
%Similar to Appendix \ref{appendix.covforCase2}, the covariance is mainly composed of covariance of Poisson random variables, such as $ \operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\} $ when $ i-1=j+2m $, which means that $\operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right)$ and $ \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right) $ are actually the same random variable as a result that they are from Poisson process during the same period of time.\\
%Let
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{12}} \triangleq {\bold E}\left(\operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right),
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%		\mathrm{E_{13}}\triangleq{\bold E}&\left(\operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right),
%	\end{aligned}
%\end{equation}
%\begin{equation}
%	\begin{aligned}
%	\mathrm{E_{14}} \triangleq	{\bold E}&\left(\operatorname{\bold Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right).
%	\end{aligned}
%\end{equation}
%\subsection{The case where $ s_j$ lies in RANDOM part}
%\subsubsection{The case that $1 \leq j \leq (\frac{1-\alpha}{2} L-2m-1) $ or $ (\frac{1+\alpha}{2} L+1)\leq j \leq \left(L-2m-1\right) $} We have $ {\bold E}\left(s_{j}s_{j+2m}\right) = \frac{1}{4}$ and $ {\bold E}\left(s_{j}s_{j+2m+1}\right) = \frac{1}{4}$ and ${\bold E}\left\{s_{j}s_{j+2m}s_{j+2m+1}\right\}=\frac{1}{8}$, since $ s_{j},s_{j+2m}$ and $s_{j+2m+1} $ lie in RANDOM part.\\
%%First, when $ s_j$ or $ s_{j+2m}$ are in RANDOM part, $\mathrm{E}$$\left\{s_{j}s_{j+2m+1}\right\}=\frac{1}{4}$, $\mathrm{E}$$\left\{s_{j}s_{j+2m}\right\}=\frac{1}{4}$, $\mathrm{E}$$\left\{s_{j+2m}s_{j+2m+1}\right\}=\frac{1}{4}$.
%For $ \left((1-\alpha)-4m-2\right) $ pairs of $ \left(i,j\right) $ with $ i-1=j+2m $, 
%\begin{equation}
%	\begin{aligned}
%%	&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%     \left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)\\
%	\mathrm{E_{12}}={\bold E}\left\{\left(2 s_{j}-1\right)\left(2 s_{j+2m+1}-1\right)\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}
%	=0,~~~\mathrm{E_{13}}=0.
%	\end{aligned}
%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		\mathrm{E_{13}}=0,
%%	\end{aligned}
%%\end{equation}
%%\begin{align}
%%	&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,\\
%%	&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\end{align}
%For $ \left((1-\alpha)-4m-2\right) $ pairs of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{14}}=0.
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $ j=\frac{1-\alpha}{2}L-2m $} We have $ s_{j+2m} $ lying in RANDOM part as well as $ s_{j+2m+1} = 1$. $ s_{j+2m+1} $ lies in $1-0$ alternate part.\\
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}=0$, $\mathrm{E_{13}}=0$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{12}}=0,
%%~~~\mathrm{E_{13}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		=0,
%%	\end{aligned}
%%\end{equation}
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)
%%	\mathrm{E_{14}}	=0,
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $(\frac{1-\alpha}{2}L-2m+1) \leq j \leq \frac{1-\alpha}{2}L$} We have $ s_{j+2m} $ and $ s_{j+2m+1} $ lying in $1-0$ alternate part with $ s_{j} $ lies in RANDOM part. Thus, $  s_{j+2m} s_{j+2m+1} =0 $.\\
%For $ 2m $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}=0$, $\mathrm{E_{13}}=0$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{12}}=0,
%%~~~\mathrm{E_{13}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		=0,
%%	\end{aligned}
%%\end{equation}
%For $ 2m $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{14}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=0,
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $ j=L-2m $} We have $ s_{j} $ and $ s_{j+2m} $ lying in RANDOM part as well as $ s_{j+2m+1} = 0$.\\
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}=0$, $\mathrm{E_{13}}=0$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{12}}=0,
%%~~~\mathrm{E_{13}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%	\end{aligned}
%%\end{equation}
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{14}}=0.
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $(L-2m+1) \leq j \leq L $} We have $ s_{j+2m} = 0$ as well as $ s_{j+2m+1} = 0$.\\
%For $ 2m $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}=0$, $\mathrm{E_{13}}=0$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{12}}=0,
%%~~~\mathrm{E_{13}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		=0,
%%	\end{aligned}
%%\end{equation}
%For $ 2m $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{14}}=0.
%%	\end{aligned}
%%\end{equation}
%\subsection{The case where $ s_j$ lies in $1-0$ alternate part} 
%\subsubsection{The case that $ \left(\frac{1-\alpha}{2} L +2\right) \leq j \leq \left(\frac{1+\alpha}{2}L-2m-1\right) $}
% We have ${\bold E}\left(s_{j}s_{j+2m}\right) = 1$ and $ {\bold E}\left(s_{j}s_{j+2m+1}\right) = 0$ with $ s_j $ not lying in boundaries.\\
%%When $ s_i$ and $ s_{i+2m}$ are in $\{1,0,...\} $ part, $\mathrm{E}$$\left\{s_{j}s_{j+2m+1}\right\}=0$, $\mathrm{E}$$\left\{s_{j}s_{j+2m}\right\}=1$, $\mathrm{E}$$\left\{s_{j+2m}s_{j+2m+1}\right\}=0$.
%For $ (\alpha L-2m-2) $ pairs of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}	=\left(- \varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)$, $\mathrm{E_{13}}= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)
%%	\mathrm{E_{12}}	=\left(- \varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	~~~\mathrm{E_{13}}= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%If $ s_j$ lies in $\{1,0,...\} $ part, we have $ \mathrm{E}\left(s_{j}s_{j+2m}\right) = 1$ and $ \mathrm{E}\left(s_{j}s_{j+2m+1}\right) = \frac{1}{4}$ when $  j = \left(\frac{1+\alpha}{2} L-2m\right) $. $ s_{j+2m}$ lies in $\{1,0,...\} $ part and $ s_{j+2m+1}$ lies in RANDOM part.
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=\left(- \varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&= -\left(\frac{k}{n}-\varepsilon \right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%For $ (\alpha L-2m-2) $ pairs of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)
%%			\mathrm{E_{14}}=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right).
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $j = \left(\frac{1+\alpha}{2} L-2m\right) $}
% We have $ s_{j}=s_{j+2m} = 0$ and $ {\bold E}\left(s_{j}s_{j+2m+1}\right) = 0$, since $ s_{j+2m}$ is the end of $1-0$ alternate part and $ s_{j+2m+1}$ lies in RANDOM part.\\
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}=0$, $\mathrm{E_{13}}=-\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2}$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%	\mathrm{E_{12}}=0,
%%	~~~	\mathrm{E_{13}}=-\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		=-\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2},
%%	\end{aligned}
%%\end{equation}
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=\left(1-\frac{k}{n}\right)\lambda_{b}$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)
%%		\mathrm{E_{14}}=\left(1-\frac{k}{n}\right)\lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $  j = \left(\frac{1-\alpha}{2} L +1\right) $} 
%We have $ s_{j}=s_{j+2m}=1$ and $ {\bold E}\left(s_{j}s_{j+2m+1}\right) = 0$, since $ s_{j} $ is the start of $1-0$ alternate part.\\
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}	=-\varepsilon\left(\lambda_{s}+\lambda_{b}\right)$, $\mathrm{E_{13}}=-\left(\frac{k}{n}-\varepsilon\right)\lambda_{b}$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)
%%	\mathrm{E_{12}}	=-\varepsilon\left(\lambda_{s}+\lambda_{b}\right),
%%	~~~\mathrm{E_{13}}=-\left(\frac{k}{n}-\varepsilon\right)\lambda_{b}.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		=-\left(\frac{k}{n}-\varepsilon\right)\lambda_{b},
%%	\end{aligned}
%%\end{equation}
%For $ 1 $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=\left(1-\frac{k}{n}\right)(\lambda_{s}+\lambda_{b})$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)
%%		\mathrm{E_{14}}=\left(1-\frac{k}{n}\right)(\lambda_{s}+\lambda_{b}).
%%	\end{aligned}
%%\end{equation}
%\subsubsection{The case that $ \left(\frac{1+\alpha}{2} L-2m+1 \leq j \leq \frac{1+\alpha}{2} L\right) $}
% We have $ {\bold E}\left(s_{j}s_{j+2m}\right) = \frac{1}{4}$ and $ {\bold E}\left(s_{j}s_{j+2m+1}\right) = \frac{1}{4}$, since $ s_{j+2m+1} $ lie in RANDOM part.\\
%For $ 2m $ pair of $ \left(i,j\right) $ with $ i-1=j+2m $, we have $\mathrm{E_{12}}=0$, $\mathrm{E_{13}}=0$.\\
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{i-1}+\lambda_{b}\right)\right),
%%%		\left(2 s_{j}-1\right) \operatorname{Poi}\left(\varepsilon\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{12}}=0,
%%~~~\mathrm{E_{13}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(\frac{k}{n}-\varepsilon\right)\left(\lambda_{s} s_{j+2m+1}+\lambda_{b}\right)\right)\right\}\right)
%%		=0,
%%	\end{aligned}
%%\end{equation}
%For $ 2m $ pair of $ \left(i,j\right) $ with $ i=j+2m $, we have $\mathrm{E_{14}}=0$.
%%\begin{equation}
%%	\begin{aligned}
%%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\right.\right.\\
%%%		&\left.\left.\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)=0,
%%\mathrm{E_{14}}=0.
%%	\end{aligned}
%%\end{equation}
%%\begin{equation}
%%	\begin{aligned}
%%		&\mathrm{E}\left(\operatorname{Cov}\left\{\left(2 s_{i}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{i}+\lambda_{b}\right)\right),\left(2 s_{j}-1\right) \operatorname{Poi}\left(\left(1-\frac{k}{n}\right)\left(\lambda_{s} s_{j+2m}+\lambda_{b}\right)\right)\right\}\right)\\
%%		&=\left(1-\frac{k}{n}\right)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right),
%%	\end{aligned}
%%\end{equation}
%By adding up components above, the mathematical expectation of covariance is,
%\begin{equation}
%\begin{aligned}
%	{\bold E}\left\{\operatorname{\bold Cov}\left(\operatorname{C}_{0,0}, \operatorname{C}_{2m, k}\right)\right\}
%%	&=(\alpha L-2 m-2)\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)\left(1-2 \frac{k}{n}\right)
%%	-\left(\frac{k}{n}-\varepsilon\right)\frac{\lambda_{s}}{2}\\
%%	&+\left(1-\frac{k}{n}\right)\lambda_{b}
%%	-\varepsilon\left(\lambda_{s}+\lambda_{b}\right)-\left(\frac{k}{n}-\varepsilon\right)\lambda_{b}+\left(1-\frac{k}{n}\right)(\lambda_{s}+\lambda_{b})\\
%	=\left(\frac{\lambda_{s}}{2}+\lambda_{b}\right)\left[\left(\alpha L -2m \right)\left(1-2\frac{k}{n}\right)+\frac{k}{n}\right]-\varepsilon\frac{\lambda_{s}}{2}.
%\end{aligned}
%\end{equation}
\end{appendices} 
%%	\begin{align}  \label{equ.deltaR_alwaysexist}
%%	-\log_2 \left[ 1+\frac{\frac{\lambda_1^2 N_1}{g_1^{(1)}}(K-1)(\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}-\frac{I\xi_i}{\lambda_i^2})}
%%	{KP_{sum}+\frac{\lambda_1^2 N_1}{g_1^{(1)}}\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}} \right]  = -\log_2 \left[ \frac{I \left( \frac{N_i}{g_i^{(1)}} + K {P_i^*}^{(1)} \right) }{KP_{sum}+\frac{\lambda_1^2 N_1}{g_1^{(1)}}\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}} \right] .
%%	\end{align}
%%	Letting $a=\frac{\lambda_1^2 N_1}{g_1^{(1)}}$ and $b=\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}$, we have $\triangle R_i = -\log_2 \left[1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]$. From Equation \eqref{equ.deltaR_alwaysexist}, it is observed that term  $1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} > 0$ due to ${P_i^*}^{(1)} \geq 0$. Then, we have
%%	\begin{align} \label{equ.First_order_partial_derivative}
%%	\frac{\partial R_i}{\partial K} = \frac{-\log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) }{(KP_{sum}+ab)^2 \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]}.
%%	\end{align}
%%	For the $i$-th sub-channel, if $(b-\frac{I \xi_i}{\lambda_i^2})<0$, we have
%%	\begin{equation}
%%	\frac{\partial \triangle R_i}{\partial K} > \frac{-\log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) }{(KP_{sum}+ab)^2} > 0.
%%	\end{equation}
%%	If $(b-\frac{I \xi_i}{\lambda_i^2})>0$, we have
%%	\begin{equation}
%%	0 > \frac{\partial \triangle R_i}{\partial K} > \frac{-\log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) }{(KP_{sum}+ab)^2}.
%%	\end{equation}
%%	Hence, we have
%%	\begin{align}\label{equ.first_order_K>1}
%%	\frac{\partial \triangle R}{\partial K} =  \sum_{i=1}^I \frac{\partial \triangle R_i}{\partial K}
%%	> \sum_{i=1}^I \frac{-\log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) }{(KP_{sum}+ab)^2}  = 0 . 
%%	\end{align}
%%	It is seen that sum-rate difference increases with $K$ for $K>1$ and 
%%	\begin{equation}
%%	\lim_{K\rightarrow \infty} \triangle R = -\log_2 \prod_{i=1}^I \left[ 1+\frac{\frac{\lambda_1^2 N_1}{g_1^{(1)}}(\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}-\frac{I \xi_i}{\lambda_i^2})}
%%	{P_{sum}} \right],
%%	\end{equation}
%%	which is an upper bound independent of $K$.
%%	
%%	Then, letting $A_i = \log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) $, the second-order partial derivative of rate difference with respect to $K$ can be written as
%%	\begin{equation}
%%	\frac{\partial^2 \triangle R_i}{\partial K^2} = \frac{A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]}
%%	+ \frac{A_i \left[ P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) \right]}{(KP_{sum}+ab)^3 \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]^2}.
%%	\label{equ.second_order_partial_derivative}
%%	\end{equation}
%%	When $K$ approaches 1, we have
%%	\begin{equation}
%%	\frac{A_i \left[ P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) \right]}{(KP_{sum}+ab)^3 \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]^2}
%%	> \frac{A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 }. \label{equ.K_approaches 1}
%%	\end{equation}
%%	For the $i$-th sub-channel, if the following formula is satisfied
%%	\begin{align}\label{equ.condition 2}
%%	&\frac{A_i \left[ P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) \right]}{(KP_{sum}+ab)^3 \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]^2}
%%	- \frac{A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 } \notag \\
%%	> & \frac{A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 } -
%%	\frac{A_i \cdot P_{sum}}{(KP_{sum}+ab)^3 \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]}, 
%%	\end{align}
%%	we have $\frac{\partial^2 \triangle R_i}{\partial K^2} > \frac{2A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 }$. Since $1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \approx 1$ when $K$ approaches to 1, Equations \eqref{equ.K_approaches 1} and \eqref{equ.condition 2} are satisfied simultaneously, leading to $\frac{\partial^2 \triangle R}{\partial K^2} = \sum_{i=1}^I \frac{\partial^2 \triangle R_i}{\partial K^2} > \sum_{i=1}^I \frac{2A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 } = 0$. As $K$ increases, $\left| \frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right| $ also increases and Equation \eqref{equ.condition 2} will not hold for some sub-channels, leading to $\frac{\partial^2 \triangle R}{\partial K^2} = \sum_{i=1}^I \frac{\partial^2 \triangle R_i}{\partial K^2} < 0$. As $K$ further increases, Equations \eqref{equ.K_approaches 1} and \eqref{equ.condition 2} are not satisfied, but $\frac{\partial^2 \triangle R}{\partial K^2} < 0$ still holds. Hence, letting $K_0$ satisfies $\frac{\partial^2 \triangle R}{\partial K^2}|_{K = K_0} = 0$, $\frac{\partial^2 \triangle R}{\partial K^2} < 0$ always holds within the range of $K>K_0$.
%%	
%%	However, it is difficult to obtain the closed form of $K_0$. Then, we give an upper bound on $K_0$. From the above analysis, $\frac{\partial^2 \triangle R}{\partial K^2} < 0$ when Equation \eqref{equ.condition 2} doesn't hold for all sub-channels. Hence, we have	    
%%	\begin{align}\label{equ.K_2ord0_cri}
%%	& A_i\left[ P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) \right] - 2A_i P_{sum} \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right]^2 \notag \\
%%	& + A_i P_{sum} \left[ 1+\frac{a(K-1)(b-\frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+ab} \right] < 0.
%%	\end{align}
%%	For the $i$-th sub-channel, it is easy to get the solution of Equation \eqref{equ.K_2ord0_cri} as 
%%	\begin{equation}
%%	K > \frac{a \left[ \frac{1}{4}b + \sqrt{\frac{9}{16} + \frac{a}{2P_{sum}}(b-\frac{I \xi_i}{\lambda_i^2}) }b - \frac{I \xi_i}{\lambda_i^2} \right]  }{a(b-\frac{I \xi_i}{\lambda_i^2}) +\left[ \frac{3}{4} - \sqrt{\frac{9}{16} + \frac{a}{2P_{sum}}(b-\frac{I \xi_i}{\lambda_i^2}) } \right] P_{sum}  }.
%%	\end{equation}
%%	We take the intersection of the solutions of all sub-channels and the upper bound of $K_0$ can be calculated by
%%	\begin{equation}\label{equ.K_0_upperbound}
%%	K_{0,ub} =  \max_{i} \left\lbrace  \frac{\frac{\lambda_1^2 N_1}{g_1^{(1)}} \left[ \frac{1}{4}\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}  + \sqrt{\frac{9}{16} + \frac{\lambda_1^2 N_1}{2g_1^{(1)}P_{sum}}(\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}-\frac{I \xi_i}{\lambda_i^2}) }\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}  - \frac{I \xi_i}{\lambda_i^2} \right]  }{\frac{\lambda_1^2 N_1}{g_1^{(1)}}(\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}-\frac{I \xi_i}{\lambda_i^2}) +\left[ \frac{3}{4} - \sqrt{\frac{9}{16} + \frac{\lambda_1^2 N_1}{2g_1^{(1)}P_{sum}}(\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}-\frac{I \xi_i}{\lambda_i^2}) } \right] P_{sum}  } \right\rbrace .
%%	\end{equation}
%%	It is worth mentioning that $\frac{\lambda_1^2 N_1}{2g_1^{(1)}P_{sum}}(\sum_{j=1}^I\frac{\xi_j}{\lambda_j^2}-\frac{I \xi_i}{\lambda_i^2})$ approaches to 0 as the SNR increases. Hence, $K_{0,ub}$ is close to 1 in high SNR environment.		
%%	
%%	
%%	\section{ proof of Theorem \ref{theorem_Kless1}} \label{appendix_Kless1}
%%	%Denote 
%%	%\begin{equation} 
%%	%R^u \triangleq -\log_2 \prod_{j=1}^N \left[ 1+\frac{\frac{\lambda_1^2 N_1}{g_1^{(1)}}(K-1)(\sum_{i=1}^N\frac{\xi_i}{\lambda_i^2}-\frac{N\xi_j}{\lambda_j^2})}
%%	%{KP_{sum}+\frac{\lambda_1^2 N_1}{g_1^{(1)}}\sum_{i=1}^N\frac{\xi_i}{\lambda_i^2}} \right].
%%	%\end{equation}
%%	According to Equation \eqref{equ.deltaR_j}, we know that $\triangle \acute{R}$ is derived from ${P_i^{*}}^{(1)}$ and ${P_i^{*}}^{(2)}$, $1 \leq i \leq I$. However, within range $0<K<K_{min}$, ${P_i^{*}}^{(2)}$ is negative if we still use equation ${P_i^{*}}^{(2)}=  \frac{P_{sum}}{I} + \frac{\lambda_1^2 N_1 }{K g_1^{(1)}} \left(\frac{1}{I} \sum_{j=1}^{I} \frac{\xi_j}{\lambda_j^2}  - \frac{\xi_i}{\lambda_i^2} \right) $. Hence, $\triangle \acute{R}$ is the ``ideal'' sum-rate difference without non-negative power constraint; and if the non-negative power constraint in Equation \eqref{equ.Poweralloc_OAM} holds, the allocated powers in some sub-channels are 0, which causes that $\triangle R \neq \triangle \acute{R}$. Moreover, since $\triangle \acute{R}$ is the ``ideal" value of $\triangle R$, it is easy to have that $\triangle R \leq \triangle \acute{R}$ within range $0<K<K_{min}$.
%%	
%%	When $0<K<1$, $K-1<0$ always holds. According to Equation \eqref{equ.First_order_partial_derivative}, if $(b-\frac{I \xi_i}{\lambda_i^2})<0$ is satisfied for the $i$-th sub-channel, we have
%%	\begin{equation}
%%	\frac{-\log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) }{(KP_{sum}+ab)^2} > \frac{\partial \triangle \acute{R}_i}{\partial K} > 0.
%%	\end{equation}
%%	If $(b-\frac{I \xi_i}{\lambda_i^2})>0$, we have
%%	\begin{equation}
%%	0 > \frac{-\log_2e \cdot a(b-\frac{I \xi_i}{\lambda_i^2})(P_{sum}+ab) }{(KP_{sum}+ab)^2} >  \frac{\partial \triangle \acute{R}_i}{\partial K}.
%%	\end{equation}
%%	Then, we have
%%	\begin{equation}\label{equ.first_order_K<1}
%%	\frac{\partial \triangle \acute{R}}{\partial K} =  \sum_{i=1}^I \frac{\partial \triangle \acute{R}_i}{\partial K} < 0.
%%	\end{equation}
%%	Hence, it is known that $\triangle \acute{R}$ decreases monotonically with $K$ within range $0<K<1$ and we have 
%%	\begin{equation}
%%	\triangle R \leq \triangle \acute{R} \leq \triangle \acute{R}|_{K=0} = \log_2 \prod_{i=1}^I \left(  \frac{\lambda_i^2}{\xi_i} \right)  + I \log_2 \left( \frac{1}{I} \sum_{j=1}^I\frac{\xi_j}{\lambda_j^2} \right).
%%	\end{equation}
%%	
%%	For the range $K_{min}<K<1$, $\triangle R =\triangle \acute{R}$ and we have $\frac{\partial \triangle R}{\partial K} =  \sum_{i=1}^I \frac{\partial \triangle R_i}{\partial K} < 0$. Meanwhile, $ P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) > 0$ always satisfies within this range. According to Equation \eqref{equ.second_order_partial_derivative}, if $(b-\frac{I \xi_i}{\lambda_i^2})<0$ is satisfied for the $i$-th sub-channel, we have
%%	
%%	\begin{equation}
%%	0 > \frac{\partial^2 \triangle R_i}{\partial K^2 }> \frac{A_i \left[2 P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) \right]}{(KP_{sum}+ab)^3} > \frac{2A_i\cdot P_{sum}}{(KP_{sum}+ab)^3}.
%%	\end{equation}
%%	
%%	If $(b-\frac{I \xi_i}{\lambda_i^2})>0$ is satisfied, we have
%%	
%%	\begin{equation}
%%	\frac{\partial^2 \triangle R_i}{\partial K^2 }> \frac{A_i \left[2 P_{sum} + a(b-\frac{I \xi_i}{\lambda_i^2}) \right]}{(KP_{sum}+ab)^3} > \frac{2A_i\cdot P_{sum}}{(KP_{sum}+ab)^3} > 0.
%%	\end{equation}
%%	
%%	Hence we have
%%	
%%	\begin{equation}\label{equ.second_order_K<1}
%%	\frac{\partial^2 \triangle R}{\partial K^2} = \sum_{i=1}^I \frac{\partial^2 \triangle R_i}{\partial K^2} > \sum_{i=1}^I \frac{2A_i\cdot P_{sum}}{(KP_{sum}+ab)^3 } = 0.
%%	\end{equation}
%%	
%%	Similarly, we have $\frac{\partial^3 \triangle R}{\partial K^3}<0$ using the same method. Thus, within range $K_{min}<K<1$, $\frac{\partial \triangle R}{\partial K}<0$, $\frac{\partial^2 \triangle R}{\partial K^2}>0$ and $\frac{\partial^3 \triangle R}{\partial K^3}<0$ always hold.
%%	
%%	\section{ proof of Lemma \ref{lemma_product_decrease}} \label{appendix.Lemma2}
%%	Let $f(x) = \log(1+x)$. Since $f(x)$ is concave in the domain $x > -1$, the inequality $f(y)\leq f(x) + f^{'}(x)(y-x) $ always holds. If $a_i$ and $b_i$ satisfy $a_i b_i \geq 0$ and $a_i+b_i>-1$, we have  
%%	\begin{align}
%%	\log(1+a_i+b_i) \leq \log(1+a_i) + \frac{b_i}{1+a_i},
%%	\end{align}
%%	where $1 \leq i \leq n$. The set $ \left\lbrace i| a_i b_i \geq 0 \right\rbrace $ can be divided into three mutually exclusive sets $ \left\lbrace i| a_i < 0, b_i \leq 0 \right\rbrace $, $ \left\lbrace i| a_i > 0, b_i \geq 0 \right\rbrace $ and $\left\lbrace i| a_i = 0 \right\rbrace $. For any $a_i < 0$ and $b_i \leq 0$, we can get $a_i > -1$ according to $a_i+b_i>-1$. Thus, $ \frac{1}{1+a_i}>1$ always holds, and we further have $ \frac{b_i}{1+a_i} \leq  b_i$. For any $a_i > 0$ and $b_i \geq 0$, we can get $0<\frac{1}{1+a_i}<1$, and then, we have $\frac{b_i}{1+a_i} \leq  b_i $. For any $a_i = 0$, we can easily get $\frac{b_i}{1+a_i} = b_i$. Hence, the above results can lead to the following inequality
%%	\begin{align}
%%	\log(1+a_i+b_i) \leq \log(1+a_i) + \frac{b_i}{1+a_i} \leq \log(1+a_i) + b_i.
%%	\end{align}
%%	If $\sum_{i=1}^n b_i=0$, we have 
%%	\begin{align}
%%	\sum_{i=1}^n \log(1+a_i+b_i) \leq \sum_{i=1}^n \log(1+a_i) + \sum_{i=1}^n b_i =\sum_{i=1}^n \log(1+a_i) ,
%%	\end{align}
%%	which can readily lead to the inequality $\prod_{i=1}^n (1+a_i+b_i) \leq \prod_{i=1}^n (1+a_i)$.
%%		
%%%	Assume $f(x_1,x_2,\cdots,x_n)=(1+x_1)(1+x_2)\cdots(1+x_n)$ and $\sum_{i=1}^n x_i=0$. The logarithm of $f(x_1,x_2,\cdots,x_n)$ can be written as $\log f(x_1,x_2,\cdots,x_n)=\sum_{i=1}^n \log(1+x_i)$. For any $x_i<0,x_j>0$, we have
%%%	\begin{align}
%%%	&\log(1+x_i-\triangle x) + \log(1+x_j+\triangle x)- \log(1+x_i)- \log(1+x_j) \notag \\
%%%	=& -[\log(1+x_i)-\log(1+x_i-\triangle x)]+\log(1+x_j+\triangle x)-\log(1+x_j)\notag \\
%%%	=& -f^{'}(\beta_i)\triangle x + f^{'}(\beta_j)\triangle x ,
%%%	\end{align}
%%%	where $\triangle x>0$ and $x_i-\triangle x>-1$. According to lagrange mean value theorem, we have $f^{'}(\beta_i) > f^{'}(\beta_j)$. Thus, for any $x_i<0,x_j>0$, 
%%%	\begin{equation}
%%%	\log(1+x_i-\triangle x) + \log(1+x_j-\triangle x)< \log(1+x_i)+ \log(1+x_j).
%%%	\end{equation}
%%%	Then, $(1+x_i-\triangle x)(1+x_j-\triangle x)<(1+x_i)(1+x_j)$ is also satisfied, which can readily lead to equation \eqref{equ.product_decrease}.
%%	
%%	\section{proof of Theorem \ref{theorem_initial_condition}}  \label{appendix.effect_of_g_N}
%%	Denote 
%%	\begin{align}
%%	\varrho_i \triangleq  \frac{\frac{\lambda_1^2 N_1}{g_1^{(1)}}(K-1)(\sum_{j=1}^I \frac{\xi_j}{\lambda_j^2} - \frac{I \xi_i}{\lambda_i^2})}{KP_{sum}+\frac{\lambda_1^2 N_1}{g_1^{(1)}}\cdot \sum_{j=1}^I \frac{\xi_j}{\lambda_j^2}}, \quad  \nu_i \triangleq \frac{\frac{\lambda_1^2 N_1}{g_1^{(1)}}(\sum_{j=1}^I \frac{\xi_j}{\lambda_j^2} - \frac{I \xi_i}{\lambda_i^2})}{P_{sum}} .
%%	\end{align}
%%	Since $\left| \varrho_i \right|$ for $1\leq i \leq I$ decreases as $\frac{g_1^{(1)}}{N_1}$ increases, $\prod_{i=1}^I (1 + \varrho_i)$ increases based on Lemma \ref{lemma_product_decrease}. According to Equation \eqref{equ.sum_rate_diff_Kless1}, upper bound $\triangle \acute{R}$ of sum-rate difference for any $0 < K < 1$ also decreases as $\frac{g_1^{(1)}}{N_1}$ increases. Assume that $\triangle \acute{R}_1$ and $\triangle \acute{R}_2$ are the corresponding upper bounds in Equation \eqref{equ.sum_rate_diff_Kless1} under two channel conditions  $\frac{g_1^{(1)}}{N_1} = \varpi_1$ and $\frac{g_1^{(1)}}{N_1} = \varpi_2$, respectively, where $(\frac{g_1}{N_1})_{min} < \varpi_1 < \varpi_2$. For any $K_{\epsilon_1, 1}$ satisfying $0 < K_{\epsilon_1, 1} < 1$, assuming that $K_{\epsilon_1, 1} = \triangle \acute{R}_1^{-1}(\epsilon_1) = \triangle \acute{R}_2^{-1}(\epsilon_2)$, we have $\epsilon_1 > \epsilon_2$. Since $\triangle \acute{R}_2$ decreases monotonically with $K$ within range $0 < K < 1$, we have $K_{\epsilon_1, 2} = \triangle \acute{R}_2^{-1}(\epsilon_1) < \triangle \acute{R}_2^{-1}(\epsilon_2) = K_{\epsilon_1, 1}$, which indicates that $K_{\epsilon}$ decreases as $\frac{g_1^{(1)}}{N_1}$ increases. Moreover, within range $K_{\epsilon} < K < 1$, $\triangle \acute{R} < \epsilon$ always holds, and such range expands as $\frac{g_1^{(1)}}{N_1}$ increases. However, from Equation \eqref{equ.sum_rate_diff_Kless1}, it is observed that $\triangle \acute{R}^u$ is independent of $\frac{g_1^{(1)}}{N_1}$. Then, since $\left| \nu_i \right|$ for $1\leq i \leq I$ decreases as $\frac{g_1^{(1)}}{N_1}$ increases, $\prod_{i=1}^I (1 + \nu_i)$ increases based on Lemma \ref{lemma_product_decrease}, and thus the upper bound of sum-rate difference in Equation \eqref{equ.upper_bound_K>1} also decreases.
%%	
%%	
%%	
%%	
%%	\section{ proof of Theorem \ref{theorem.dmin_diff_power_allocation}} \label{appendix.dmin_diff}
%%	Letting $\mathbf{A^*}=sqrt(diag(\mathbf{p^*}))$ and $\mathbf{A}^{map}=sqrt(diag(\mathbf{p}^{map}))$, we first consider the following normalized MED difference, 
%%	\begin{align}
%%	&\left| 1 - \frac{d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) }{d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^m )}  \right| 
%%	\leq  \left| 1 - \frac{d_{min}^2(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) }{d_{min}^2(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^m )}  \right|  
%%	=  \left| 1 - \frac{\|\mathbf{Z}\mathbf{H}\mathbf{A}^{map}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2 }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2}  \right| \notag \\
%%	\leq & \max \left\{\left| 1 - \frac{\|\mathbf{Z}\mathbf{H}\mathbf{A}^{map}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2 }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2}  \right|, \left| 1 - \frac{\|\mathbf{Z}\mathbf{H}\mathbf{A}^{map}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2 }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2}  \right| \right\},
%%	\end{align}
%%	where
%%	\begin{align}
%%	&\left| 1 - \frac{\|\mathbf{Z}\mathbf{H}\mathbf{A}^{map}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2 }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2}  \right| 
%%	=  \frac{\left| \sum_{i =1 }^N \frac{|h_i|^2}{N_i}(p_i^* - p_i^{map})|\mathbf{s}_m^m(i)-\mathbf{s}_{\hat{m}}^m(i)|^2 \right| }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2} \notag \\
%%	\leq & \frac{ \sum_{i =1 }^N \frac{|h_i|^2}{N_i} |p_i^* - p_i^{map}|\cdot |\mathbf{s}_m^m(i)-\mathbf{s}_{\hat{m}}^m(i)|^2  }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2} \notag \\
%%	\leq & \frac{ \left( \sum_{i =1 }^N \frac{|h_i|^4}{N_i^2}  |\mathbf{s}_m^m(i)-\mathbf{s}_{\hat{m}}^m(i)|^4\right) ^\frac{1}{2} \cdot \left( \sum_{i =1 }^N |p_i^* - p_i^{map}|^2 \right) ^\frac{1}{2} }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2} \notag \\
%%	\leq & \frac{  (\sum_{i =1 }^N \frac{|h_i|^2}{N_i}  |\mathbf{s}_m^m(i)-\mathbf{s}_{\hat{m}}^m(i)|^2 ) \cdot \left\| \mathbf{p}^* - \mathbf{p}^{map} \right\|_2  }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2} \notag \\
%%	= & \frac{  \|\mathbf{Z}\mathbf{H}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2 \cdot \left\| \mathbf{p}^* - \mathbf{p}^{map} \right\|_2  }{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2}.
%%	\end{align}
%%	Similarly, we can obtain the upper bound of $\left| 1 - \|\mathbf{Z}\mathbf{H}\mathbf{A}^{map}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2 /\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2  \right| $. 
%%	Hence, the upper bound of $\left| 1 - d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) /d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^m )  \right|$ can be written as
%%	\begin{equation}
%%	\left| 1 - \frac{d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) }{d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^m )}  \right| \leq \left\| \mathbf{p}^* - \mathbf{p}^{map} \right\|_2 \cdot \max \left\{ \frac{  \|\mathbf{Z}\mathbf{H}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2}{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m)\|_2^2}, \frac{  \|\mathbf{Z}\mathbf{H}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2}{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}(\mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m)\|_2^2}\right\}.
%%	\end{equation}
%%	Since the normalized MED difference $\left| 1 - d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^{m} ) / d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^* ) \right|$ satisfies
%%	\begin{equation}
%%	\left| 1 - \frac{d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) }{d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^* )}  \right| \leq \max \left\{ \left| 1 - \frac{d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) }{d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^m )}  \right|, \left| 1 - \frac{d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^* ) }{d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^* )}  \right| \right\},
%%	\end{equation}
%%	we have
%%	\begin{equation}
%%	\left| 1 - \frac{d_{min}(\mathbf{H}, \mathbf{p}^{map}, \mathcal{C}^m ) }{d_{min}(\mathbf{H}, \mathbf{p}^*, \mathcal{C}^* )}  \right| \leq \left\| \mathbf{p}^* - \mathbf{p}^{map} \right\|_2 \cdot \max_{\tilde{\mathbf{s}} \in \mathbf{s}_d} \left\{ \frac{  \|\mathbf{Z}\mathbf{H}\tilde{\mathbf{s}}\|_2^2}{\|\mathbf{Z}\mathbf{H}\mathbf{A^*}\tilde{\mathbf{s}}\|_2^2}\right\},
%%	\end{equation}
%%	where $\mathbf{s}_d$ is the set of $ \left\{ \mathbf{s}_o^*-\mathbf{s}_{\hat{o}}^*, \mathbf{s}_o^m-\mathbf{s}_{\hat{o}}^m, \mathbf{s}_m^*-\mathbf{s}_{\hat{m}}^*,  \mathbf{s}_m^m-\mathbf{s}_{\hat{m}}^m \right\}$. 
%%	%Term $\|\mathbf{Z}\mathbf{H}\mathbf{A^*}\tilde{\mathbf{s}}\|_2^2 = 0$ if $\mathbf{A^*}\tilde{\mathbf{s}} = \mathbf{0}$, which is happened only when the activated sub-channels under $\mathbf{p}^*$ and $\mathbf{p}^{map}$ are all different. However, the threshold $\tau_{s}$, which determines whether two positions are classified into one category in power allocation map, is generally not very large and therefore the above situation does not occur, which indicates that term $\|\mathbf{Z}\mathbf{H}\mathbf{A^*}\tilde{\mathbf{s}}\|_2^2$ is finite. Meanwhile, as term $\|\mathbf{Z}\mathbf{H}\tilde{\mathbf{s}}\|_2^2$ is finite, $\max_{\tilde{\mathbf{s}} \in \mathbf{s}_d} \left\{    \|\mathbf{Z}\mathbf{H}\tilde{\mathbf{s}}\|_2^2 / \|\mathbf{Z}\mathbf{H}\mathbf{A^*}\tilde{\mathbf{s}}\|_2^2\right\}$ is finite.
%%	
%%	\section{ proof of Theorem \ref{theorem.dmin_diff_nonuniform_linkgain}} \label{appendix.dmin_diff_nonuniform}
%%	According to the definition of MED, we have
%%	\begin{align}  \label{equ.deltaH_upperbound}
%%	& 1 - \frac{d_{min}(\mathbf{H}^{(2)}, \mathbf{p}, \mathcal{C}^{*,(1)} ) }{d_{min}(\mathbf{H}^{(2)}, \mathbf{p}, \mathcal{C}^{*,(2)} )}  
%%	=  1 -\frac{\|\mathbf{Z}(\alpha \mathbf{H}^{(1)} + \Delta \mathbf{H})\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2 }{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & 1 -\frac{\|\mathbf{Z} \alpha \mathbf{H}^{(1)} \mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H}\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & 1 -\frac{\|\mathbf{Z} \alpha \mathbf{H}^{(1)} \mathbf{A} (\mathbf{s}_m^{(1)}-\mathbf{s}_{\hat{m}}^{(1)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H}\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & 1 -\frac{\|\mathbf{Z} \alpha \mathbf{H}^{(1)} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H}\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & 1 -\frac{\|\mathbf{Z} \mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H}\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & 1 -\frac{\|\mathbf{Z} \mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 - \|\mathbf{Z} \Delta \mathbf{H}\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & \frac{ \|\mathbf{Z} \Delta \mathbf{H} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 + \|\mathbf{Z} \Delta \mathbf{H}\mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}  \notag \\
%%	\leq & \frac{ \|\Delta \mathbf{H} \|_F(\|\mathbf{Z} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 + \|\mathbf{Z} \mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2)}{\|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2}.
%%	\end{align}
%%	In general, terms $(\|\mathbf{Z} \mathbf{A} (\mathbf{s}_m^{(2)}-\mathbf{s}_{\hat{m}}^{(2)})\|_2 $, $ \|\mathbf{Z} \mathbf{A} (\mathbf{s}_o^{(1)}-\mathbf{s}_{\hat{o}}^{(1)})\|_2) $ and $ \|\mathbf{Z}\mathbf{H}^{(2)} \mathbf{A} (\mathbf{s}_o^{(2)}-\mathbf{s}_{\hat{o}}^{(2)})\|_2$ are finite.
%%	
%%	
%%\end{appendices} 

==> Sec1_Introduction.tex <==


\section{Introductions}
%\subsection{Background}
%Wireless optical communication (free space optical communication) technology, compared with the traditional radio communication, effectively avoid the problem of insufficient the channel capacity, insufficient spectrum resources and serious electromagnetic interference; Compared with optical fiber communication, it can also cope with the problem that wired optical communication system is not free enough and has poor mobility. Among them, ultraviolet communication not only has the above advantages of wireless optical communication, compared with other bands of optical communication, ultraviolet light due to its own scattering characteristics, carrier propagation path is more diverse, so ultraviolet communication has been widely concerned.
Terminal positioning has a wide variety of applications, relying on frequency, time and spatial information. Timing-based positioning techniques rely on the measurements of flying times of signals between nodes. Among them, time difference of arrivals (TDOA) techniques are effective in locating a source based on intersections of hyperbolic curves defined by the arrival time differences of received signal and are further improved with bias reduction \cite{301830,6151186}. Solution and performance analysis of geolocation by TDOA are investigated \cite{259534,4682575}. Work \cite{5778025} develops an linear solution that estimate the target location based on TDOA technique for ultra-wide band (UWB) localization. Work \cite{1323254} proposes an algebraic solution for the position and velocity of a moving terminal using TDOA of signals received at a number of receivers. Geolocation based on biased range estimates is proposed \cite{6151850}. A TDOA-based optical wireless indoor localization approach is proposed using light emitting diodes (LEDs) and the performance is demonstrated \cite{6131130}.
%Due to the scattering of ultraviolet (UV) signals in the atmosphere, UV communication can be applied to the scenario where the transmitter and receiver cannot be perfectly aligned.

On the other hand, optical wireless communication (OWC) refers to transmission in unguided propagation media through optical carriers, i.e., visible, infrared (IR) and ultra-violet (UV) band \cite{6844864}. In comparison to radio-frequency (RF) counterparts, the OWC link shows potential immunity to electromagnetic interference and does not have electromagnetic radiation \cite{1159099,5175684,6165319,6458971}. It also provides a high reuse factor, an inherent security, and robustness to electromagnetic interference \cite{4063386}. Laser-based free-space optical (FSO) systems are also appealing for a wide range of applications, for example, an envisioned campus connectivity scenario where inter-building connections are enabled by high data rate FSO links or high quality video surveillance. The monitoring of a city can be made possible by FSO links \cite{4063386,938713,1299334}. The UV-C band is essentially solar blind, where most solar radiation is getting absorbed by the ozone layer in the upper atmosphere, which results in an almost noiseless transmission channel \cite{1527982}. Hence, a photon detector can approach quantum-limited photon counting detection performance \cite{8641355}. Besides, line-of-sight (LOS) configurations in the UV-C band have additional desirable characteristics compared to conventional optical wireless networks operating outside this band.

 Due to almost negligible background radiation in the UV spectrum close to the earth surface, high-sensitivity photon-level detection can be developped based on multi-stage amplification \cite{1527982,10.1117/12.582002}, for example using a photomultiplier tube (PMT). The channel characteristics of UV communication have been demonstrated experimentally in \cite{5342313,Xiao2011NonlineofsightUS,6923957,Liao2015LongdistanceNU,Borah2021SingleAD,9295804}, where Monte-Carlo approach is adopted to trace the transmission path of a photon experiencing random scattering and attenuation events. Relay communication protocols have been designed and studied in \cite{6877718,8275030,7830279}. In \cite{5599260}, generalized maximum likelihood sequence detection has been investigated. To increase the detection sensitivity, work \cite{7112175,7047703} studied the signal detection with receiver diversity. Experimental work on long-distance channel is introduced in \cite{6923957}. In \cite{8332484}, the throughput of 1Mbps has been demonstrated via receiver diversity over 1 km. Work \cite{2022arXiv220801559Y} proposes an upper bound on the synchronization mean squared error of an OWC system with a photon-counting receiver.

In recent years, the application of optical wireless transmission for positioning has attracted much attention. Various algorithms and systems for visible light positioning (VLP) have been proposed \cite{8322671,8121297,7394267,8533834,7859314}. For example, a positioning system for underwater terminals is proposed based on the underwater wireless optical code division multiple access (CDMA) network \cite{7928991}. In work \cite{10092387}, a full-duplex asymmetric underwater optical wireless communication and positioning (UOWC-UOWP) system for future underwater wireless sensor network (UWSN) is proposed. Researchers propose a visible light communication (VLC) -based ID-estimation and LED-tracking method for indoor positioning contexts \cite{7275471}. For UV band, researchers present a probabilistic fire location estimation in indoor fire environments by fusing two rotary UV sensors \cite{9158795}. However, terminal positioning based on UV transmission needs to be explored.
%Among practical system design, accurate framework synchronization is crucial for the subsequent signal detection. Work \cite{5306425} has studied the use TCH sequences for synchronization. Two new methods for constructing sets of zero-correlation zone (ZCZ) sequences are proposed in \cite{1273669}. These sequence sets have a large ZCZ that can increase the tolerable range of synchronous gap. The maximum-likelihood symbol synchronization statistic is derived from noisy observations of randomly modulated on-off-keying data for the direct-detection optical channel in \cite{1096823}. Approximations to the optimal statistic are introduced and compared to obtain a good compromise between implementation complexity and performance. Work \cite{293680} has studied symbol synchronization and sequence detection for random overlapped pulse position modulation (OPPM) sequences with maximum-likelihood algorithms operating on both hard and soft data. For channels utilizing OPPM signaling, work \cite{335965} has introduced modulation codes and joint synchronization and detection algorithms for joint estimates of symbol boundaries and transmitted symbols. A timing synchronization scheme based on Gold sequences modulated on a single subcarrier for orthogonal frequency-division multiple access passive optical network (OFDMA-PON) has been proposed in \cite{7829292}. The synchronization sequence optimization for UV communication has been preliminarily addressed for pulse-based communication \cite{8855803}. However, for UV source with constant peak power output, for example, UV LED, the synchronization sequence optimization has not been addressed.

%Frame synchronization employed in communication systems is to find valid data in a transmission by inserting a fixed data pattern. Binary sequence with perfect auto-correlation has been studied in \cite{Arasu2011SequencesAA}. There are periodical sequences' detection in a bit stream for synchronization \cite{1094813}. Researchers proposed a extension of joint frame synchronization of MIMO-OFDM systems \cite{4401715}. Rather than traditional synchronization techniques that employed the “same” fixed pattern, perfect punctured binary sequence pairs \cite{7042838} are applied to a new synchronization scheme \cite{article}. Mismatched filtering is introduced in \cite{1214826}, where the transmitter and the sender can use different sequences as a sequence pair. Such pairs attracted a lot of researchers owing to correlation properties.

%High speed communication over long distances \cite{8332484} challenges the reliability and accuracy of synchronization processes. Locating the starting moment of frame header successfully benefits accurate channel estimation and decoding. Mostly, m-sequence or Gold sequence is used as the synchronization sequence in NLOS UV scattering communication systems. Starting from m-sequence, researchers propose to optimize the frame synchronization sequence for the Z channel in Long-range NLOS ultraviolet communication \cite{8855803}. Most researches on frame synchronization sequence is at the symbolic level. So estimation offset within the duration of a symbol can still exist, which may even cause the transmission failure when the signal - noise condition is poor.

%Synchronization relies on the correlation of pulse numbers and the pretreated sequence \cite{8332484}. Our work combined with UV scattering communication systems aim to locate the moment when photons'arriving corresponding to the first symbol starts more precisely. 

This work aims to design a positioning system by UV transmission under photon-level signal detection, assuming on-off keying (OOK) modulation using UV LEDs. The positioning is based on TDOA principle. We utilize the coordinates of the known transmitters to locate the unknown receiver, and time division transmission of synchronization sequence is applied. Our work investigates the positioning error via decomposing it into two parts. The theoretical average error matches well with the simulation results. We also conduct real-time hardware realization of the TDOA-based positioning system using Field Programmable Gate Array (FPGA), which is evaluated via outdoor real-time experiments. Experimental results match well with the theoretical and simulation results. The positioning accuracy can be further improved when the clock alignment error can be reduced at the transmitters.

%\subsection{Organization}
 The remainder of this paper is organized as follows. In Section \ref{sec.system_model}, the positioning model and TDOA principle are introduced. In Section \ref{Transmittion scheme}, we decompose the timing error into two parts, the transmitter-side synchronization error and receiver-side synchronization error, and analyze each part. In Section \ref{Theoretical fitting and simulation verification}, simulation results are obtained to verify the theoretical average positioning error. In Section \ref{Outdoor Location Experiment}, we introduce the real-time hardware realization, as well as the experimental results in two outdoor real-time experiments on the university playground and a larger lawn, where the experimental results match well with the theoretical average error. Finally, Section \ref{section.conclusion} concludes this work.


%\textcolor{ColorRed}{Currently, intelligent terminals are becoming more and more universal. They not only need to provide positioning, tracking and other sensing services, but also need to provide high-speed communication service \cite{qi2020integrated, de2021convergent}. 
%However, with the development of communication technologies, the demand for spectrum resource is increasing. Such trend calls for high-frequency spectrum like millimeter wave (mmWave) and Tera Hertz (THz) \cite{6515173, 6005345}. In this work, we mainly consider the use of mmWave. Compared with sub-6GHz communication, mmWave communication can occupy wider spectrum resource (30-300 GHz) to guarantee high-speed transmission \cite{8344116}. On the other hand, orbital angular momentum (OAM), as a new degree of freedom, is applied to mmWave systems to further increase the transmission rate \cite{7968418, mmWaveOAM2014, ren2017line, 7919278, Travelingwave2015}. }

%\textcolor{ColorRed}{
%Due to the characteristics of beam diffusion and coaxial transmission, OAM is only suitable for short-range line-of-sight (LOS) communication \cite{ren2017line, yan201632, sasaki2018experiment, zhang2016orbital}. Moreover, higher spectrum will lead to larger propagation and penetration loss \cite{8207426, liu2016line,8046024}, which further limits the application to short-range LOS environment.
%In most existing mmWave systems, data processing is performed only in a single narrow spectrum \cite{7445130, 7959626}, and the advantage of abundant mmWave spectrum is not fully utilized \cite{8241348, 8252751}. Beneficial from the large link losses, mmWave systems can aggregate the licensed or unlicensed broad spectrum with small external interference to increase transmission rate.
%In general, broad spectrum communication is combined with wavelength division multiplexing (WDM) technology, which adopts multiple carrier wavelengths to transmit data streams \cite{8765239, 8910608, 8928550, 8403734}. }
%
%%With the advent of technologies such as virtual reality (VR) and augmented reality (AR), the demand for high communication rate is increasing. Such trend calls for high-frequency spectrum like millimeter wave (mmWave) and Tera Hertz (THz) \cite{6515173, 6005345}. Compared with sub-6GHz communication, mmWave communication can occupy wider spectrum resource (30-300 GHz) to guarantee high-speed transmission \cite{8344116}. However, higher spectrum will lead to larger propagation and penetration loss \cite{8207426, 7547944,8046024}, which limits the application to short-range line-of-sight (LOS) communication.
%%In most existing mmWave systems, data processing is performed only in a single narrow spectrum \cite{7445130, 7959626}, and the advantage of abundant mmWave spectrum is not fully utilized \cite{8241348, 8252751}. Beneficial from the large link losses, mmWave systems can aggregate the licensed or unlicensed broad spectrum with small external interference to increase transmission rate.
%%In general, broad spectrum communication is combined with wavelength division multiplexing (WDM) technology, which adopts multiple carrier wavelengths to transmit data streams \cite{8765239, 8910608, 8928550, 8403734}. In this work, we consider the use of mmWave, while the main results can be extended to other LOS spectrum, such as THz.
%
%%Based on the results of some indoor mmWave channel measurements, 
%
%\textcolor{ColorRed}{
%For mmWave spectrum communication in sparsely scattered environment, such as conference room and workshop, the influence of multi-path is relatively limited and the LOS path is dominant \cite{wang2018survey}. Meanwhile, the mmWave propagation shows a apparent quasi-optical property according to some experimental measurement results \cite{maltsev2009experimental, maltsev2010statistical}. Hence, the mmWave short-range LOS link can be considered as a pure LOS channel, also called determined channels \cite{liu2016line}. Based on the above feature, the link conditions of mmWave communication in short-range LOS environment are only related to the positions of transmitter and receiver \cite{chen2020multi}. Generally, high accuracy positioning is necessary for some short-range intelligent systems, such as industrial internet and indoor robot. And if OAM is adopted, this position information can be used to align the receiving antenna axis with transmitting antenna axis. Certainly, the systems can directly utilize OAM signals to locate and communicate \cite{chen2020multi, chen2018beam}. }
%
%\textcolor{ColorRed}{
%Motivated by the quasi-static feature and positioning-communication integration, we attempt to configure the communication system based on transceiver's position. Due to the stable gains for short-range LOS links, the optimal system parameters are determined when the position information is obtained. Hence, we construct a look-up table, which is named as map method, to store the system parameters of all interested positions \cite{8865431}. Adopting map-assisted approach has two potential advantages: (1) For the system whose positioning service is active, the transmitter and receiver always have position information. If a communication request appears, the system can directly configure the transmitter and receiver by adopting the parameters stored in the map. Since that there is no need for the processes of channel estimation, channel feedback and online optimization, the delay of initial communication establishment will be reduced a lot. (2) The system can solve some computationally intensive optimization problems offline and store the optimization results into the map, which significantly relaxes the online computational pressure.  }
%
%\textcolor{ColorRed}{
%Obviously, the positional quantization will mainly affect the system performance \cite{8307766}. High quantization accuracy can improve the system performance, but will increase the storage and search complexity. Therefore, it is necessary to simplify the map on a certain performance loss tolerance. And it can be expected that after quantization with certain distortion threshold, there are only a few patterns stored in the map. }
% 
%
%%On the other hand, orbital angular momentum (OAM), as a new degree of freedom, is applied to mmWave systems to further increase the transmission rate \cite{7968418, mmWaveOAM2014, 7880700, 7919278, Travelingwave2015}. OAM utilizes spatial distribution of helical phase front $e^{-jl\phi}$, where $\phi$ is the transverse azimuthal angle and $l$ is the OAM mode number \cite{Allen1992}. Moreover, different OAM modes $l$ are mutually orthogonal, allowing simultaneous and coaxial transmission to achieve higher spectral efficiency. In order to generate OAM beams, spiral phase plates (SPP) antenna and uniform circular array (UCA) are widely used in OAM multiplexing systems \cite{mmWaveOAM2014,7880700, 7797488, 8247288}. In addition, as a new kind of OAM antenna, circular traveling-wave antenna is attracting extensive attention \cite{Travelingwave2015, 7014288}. Compared with SPP and UCA, the structure of circular traveling-wave antenna is simpler, where only one single antenna can coaxially generate and transmit multiple different OAM beams. At the receiver, the UCA can detect multiple OAM modes coaxially. 
%
%%Considering the mmWave WDM with different OAM modes under LOS scenario, the same transmission distance over orthogonal links leads to the link gain correlation  \cite{8307766}. Such correlation does not exist for sub-6G spectrum with dispersed transmission, and can limit the optimal transmission modes to only a small fraction in the entire set of possible modes. Moreover, due to the stable gain for LOS link, map-based approach can be adopted to store the optimal transmission modes into the points of map \cite{8865431}. It can be expected that after quantization with certain distortion threshold, there are only a few modes stored in the map. 
%
%\textcolor{ColorRed}{
%This work considers the mmWave WDM with different OAM modes under short-range LOS scenario. We mainly focus on two issues: power allocation, which stems from channel capacity perspective, and constellation design, which primarily for improving the detection performance. Considering map-assisted communication systems, we concern that the performance loss caused by position clustering in the map. More specifically, we analyze the metric loss of each issue when the system lies at a certain position but adopts the configuration parameters of another position. For power allocation, we investigate the feasibility of using one power allocation scheme for different receiver locations. Within regions only having plane wave ($l=0$), we characterize the sum-rate difference under uniform link gain ratio, and figure out that the mmWave WDM system can employ fixed power allocation due to high signal to noise ratio (SNR) in short-range LOS scenario. Combining theoretical analyses with numerical results, we also figure out that there are a few power allocation schemes for the regions multiplexing several OAM modes, which enables the representation of power allocation using a few patterns in a map. Then, we consider the high-dimensional constellation design using minimum Euclidean distance (MED) as the performance criterion. To characterize the possibility of assigning few constellation sets to the entire interested positions, we prove that for any position 2, the normalized MED difference of using the constellation of position 1 can be sufficiently small if the channel matrices of positions 1 and 2 are sufficiently close to be proportional. Thus, a fixed constellation can be adopted for plane wave ($l=0$) only regions due to the uniform link gain ratio. The claim of only a few constellation patterns is supported by the numerical results. }
%
%%This work investigates the power allocation and constellation design of mmWave WDM with different modes in short-range LOS environment. We treat plane wave as a special case of OAM with mode zero. For power allocation, we investigate the feasibility of using one power allocation scheme for different receiver locations. For plane wave, we characterize the sum-rate difference under uniform link gain ratio and figure out that the mmWave WDM system can employ fixed power allocation within high signal to noise ratio (SNR). We also figure out that there are a few power allocation schemes for the region with higher-order OAM modes, which enables the representation of power allocation using a few modes in a map. Then, we consider the high-dimensional constellation design using minimum Euclidean distance (MED) as the performance criterion. To characterize the possibility of using few constellation sets to generate high dimensional constellations, we prove that for any position 2, the normalized MED difference of using the constellation of position 1 can be sufficiently small if the channel matrices of positions 1 and 2 are sufficiently close to be proportional. Thus, a fixed constellation can be adopted for plane wave due to the uniform link gain ratio. The claims of only a few power allocation modes and constellation sets are supported by the numerical results.

%The remainder of this paper is organized as follows. \textcolor{ColorRed}{ In Section \ref{sec.system_model}, we provide the system model, elaborate the features of OAM beams and display the configuration process of map-assisted systems. In Section \ref{section.pow_alloc}, we characterize the power allocation patterns of the region only having plane wave and the region multiplexing several OAM modes, and demonstrate that there may be only a few power allocation patterns especially under high SNR scenario.} In Section \ref{section.Cons_design}, we investigate the high dimensional constellation design, and figure out that the same link gain ratio leads to the same constellation, and that the constellation design can be represented by only a few constellation sets in the map. Finally, Section \ref{section.conclusion} concludes this paper.


==> Sec2_SystemModel.tex <==
%\graphicspath{{figures/Fig_SysModel/}}
%\graphicspath{{figure_yu/FigModel/}}

\section{Positioning Model} \label{sec.system_model}
The arrival time difference of the signal can be accurately recorded through synchronization process, based on which the terminal positioning can be achieved.
%\textcolor{ColorBlack}{
\subsection{The TDOA-Based Positioning Protocol}
    Consider 2-dimensional positioning, while 3-dimensional positioning can be derived in a similar fashion. Assume that transmitters A, B and C are three separate anchor points, which send signals to receiver R, as shown in Fig. \ref{TDOA}. The three transmitters are aligned via an unified clock in the form of pulse per second (PPS) from a satellite timing system. The transmitters send synchronization signals to the receiver under an unified clock in a time-division manner at fixed time interval $T$. The time-division transmission is controlled by $10MHz$ square wave generated by an atomic clock drived by the PPS signal. Based on the synchronization of pilots from the three transmitters, the receiver can obtain the time difference of arrival, from which the receiver location can be estimated.
    \begin{figure*}[htbp]
    	\centering
    	\includegraphics[width=4.5in]{TDOA.pdf}
    	\caption{$\ $Schematic diagram of TDOA principle.} \label{TDOA}
    	%    	\vspace{-1.0cm}%%压缩图片后间隔
    \end{figure*}
    
    Assume that the transmitters send synchronization signals via OOK modulation. Due to extremely weak light intensity, the received signal can be characterized by discrete photoelectrons, and the number of detected photoelectrons during a certain duration follows Poisson distribution. To remove the inter-transmitter interference, assume that $T$ is longer than the synchronization length, such that the signals received by the receiver from different transimitters will not overlap. Let $\lambda_{s, A}$ and $\lambda_b$ denote the mean numbers of detected photoelectrons for the signal from transmitter A and background radiation components, respectively. Assume that the three transmitters adopt the same synchronization sequence $\{s_i, 1 \leq i \leq L\}$, where $L$ is the synchronization sequence length. Let $s_i$ denote the $i^{th}$ symbol of pilot sequence and $N_{i,A}$ denote the number of received photoelectrons from the $i^{th}$ symbol, satisfying
    \begin{align} \label{equ.Poisson_channel}
    	P(N_{i,A} = u \mid s_i=1) &= \frac{(\lambda_{s, A}+\lambda_b)^{u}}{{u}!}e^{-(\lambda_{s,A}+\lambda_b)},\\
    	P(N_{i,A} = u \mid s_i=0) &= \frac{\lambda_b^{u}}{{u}!}e^{-\lambda_b}.
    \end{align} 
    For transmitter B, we have
    \begin{align} \label{equ.Poisson_channel2}
    	P(N_{i,B} = u \mid s_i=1) &= \frac{(\lambda_{s, B}+\lambda_b)^{u}}{{u}!}e^{-(\lambda_{s,B}+\lambda_b)},\\
    	P(N_{i,B} = u \mid s_i=0) &= \frac{\lambda_b^{u}}{{u}!}e^{-\lambda_b}.
    \end{align} 
   Similarly for transmitter C, we have
   \begin{align} \label{equ.Poisson_channel3}
	  	P(N_{i,C} = u \mid s_i=1) &= \frac{(\lambda_{s, C}+\lambda_b)^{u}}{{u}!}e^{-(\lambda_{s,C}+\lambda_b)},\\
	  	P(N_{i,C} = u \mid s_i=0) &= \frac{\lambda_b^{u}}{{u}!}e^{-\lambda_b}.
   \end{align} 

    Let $T_s$ denote the symbol duration. In this work, each symbol duration is divided into $n$ chips with duration $T_c = \frac{T_s}{n}$. For a certain chip index $t$, the number of pulses in that chip is denoted as $ N_{t,A} $. Let ${\hat t}_{Astart}$ denote the starting chip index estimate of the synchronization sequence. The synchronization solution is formulated by finding the following start index
    \begin{equation}
    	\begin{aligned} \label{equ.auto-correlation}
    		{\hat t}_{Astart}&=\arg \max _{t_{Astart}}\left\{\sum_{i=1}^{L}\left\{u_{i,A}^{t_{Astart}} \times\left(2 s_{i}-1\right)\right\}\right\},\\
    	\end{aligned}
    \end{equation}
    where
    \begin{equation}
    	\begin{aligned} \label{equ.n}
    		u_{i,A}^{t_{Astart}}&=\sum_{j=0}^{n-1}N_{t_{Astart}+n\times (i-1) +j,A}~,
    	\end{aligned}
    \end{equation}
denotes the number of pulses correlated with symbol $ s_{i} $ based on start chip index $ t_{Astart} $, and symbol $ s_{i} $ is transformed to $ \left(2 s_{i}-1\right) $ belonging to $ \{-1,1\} $ for correlation. Maximum correlation peak criterion is adopted. $ \hat{t}_{Astart} $ is regarded as the time when the synchronization signal reaches the receiver. Similarly, we have
   \begin{equation}
    	\begin{aligned} \label{equ.auto-correlation2}
    		{\hat t}_{Bstart}&=\arg \max _{t_{Bstart}}\left\{\sum_{i=1}^{L}\left\{u_{i,B}^{t_{Bstart}} \times\left(2 s_{i}-1\right)\right\}\right\},\\
    	\end{aligned}
    \end{equation}
	\begin{equation}
		\begin{aligned} \label{equ.auto-correlation3}
			{\hat t}_{Cstart}&=\arg \max _{t_{Cstart}}\left\{\sum_{i=1}^{L}\left\{u_{i,C}^{t_{Cstart}} \times\left(2 s_{i}-1\right)\right\}\right\}.\\
		\end{aligned}
	\end{equation}

\subsection{Positioning Algorithm: TDOA}
    TDOA measures the arrival time difference of signals from the transmitters.    
%    Consider the receiver in a UV scattering communication system with OOK modulation. Due to extremely weak light intensity, the received signal can be characterized by discrete photoelectrons and the number of detected photoelectrons during a certain duration follows Poisson distribution. Under the premise of protection interval, the signals received by the receiver from different transimitters will not overlap. So the synchronization only interferes with background noise. $\lambda_s$ and $\lambda_b$ denote the mean numbers of detected photoelectrons for the signal and background radiation components, respectively. Let $s_i$ denote the $i^{th}$ symbol and $N_i$ denote the number of received photoelectrons from the $i^{th}$ symbol, satisfying
%    \begin{align} \label{equ.Poisson_channel}
%    	P(N_i = n_i \mid s_i=1) &= \frac{(\lambda_s+\lambda_b)^{n_{i}}}{{n_{i}}!}e^{-(\lambda_s+\lambda_b)},\\
%    	P(N_i = n_i \mid s_i=0) &= \frac{\lambda_b^{n_{i}}}{{n_{i}}!}e^{-\lambda_b}.
%    \end{align} 
%    
%    Referring to \cite{8332484}, let $\{s_{i}:1\leq i \leq L\}$ denote the synchronization sequence, where $L$ is the length. Let $T_s$ denote the symbol duration. For the convenience of subsequent analysis, we assume that $T_s = 1$ is a unit of time. In this work, the received signal is divided into $n$ chips with duration $T_c = \frac{T_s}{n}$. For a certain chip index $t$, the number of pulses in that chip is denoted as $ N_{t} $. Let ${\hat t}_{start}$ denote the starting chip index estimate of the synchronization sequence. The synchronization solution is formulated by the following problem,
%    \begin{equation}
%    	\begin{aligned} \label{equ.auto-correlation}
%    		{\hat t}_{start}&=\arg \max _{t_{start}}\left\{\sum_{i=1}^{L}\left\{u_{i}^{t_{start}} \times\left(2 s_{i}-1\right)\right\}\right\},\\
%    	\end{aligned}
%    \end{equation}
%    where
%    \begin{equation}
%    	\begin{aligned} \label{equ.n}
%    		u_{i}^{t_{start}}&=\sum_{j=0}^{n-1}N_{t_{start}+n\times (i-1) +j}~,
%    	\end{aligned}
%    \end{equation}
%    denotes the number of pulses correlated with symbol $ s_{i} $ based on start chip index $ t_{start} $, and symbol $ s_{i} $ is transformed to $ \left(2 s_{i}-1\right) $ belonging to $ \{-1,1\} $ for correlation. The maximum correlation peak criterion is adopted. $ t_{start} $ is regarded as the time when the synchronization signal reaches the receiver.
Assume that the arrival time instants of the synchronization signal from the three transmitters are ${t}_A$, ${t}_B$ and ${t}_C$. The difference of flying time can be obtained accordingly considering the transmission instants from the three transmitters. Let $t_{BA}$ denote the flying time difference between signals from B and A, and $t_{CB}$ denotes the flying time difference between signals from C and B. The positioning is based on the following property
    
%    \begin{figure}[htbp]
%    	\centering
%    	\includegraphics[width=2.5in]{TDOA}
%    	\caption{$\ $Schematic diagram of TDOA principle.} \label{TDOA}
%%    	\vspace{-1.0cm}%%压缩图片后间隔
%    \end{figure}

\begin{equation}\label{d_diff}
	\begin{aligned} 
		r_{21}&=r_2-r_1=c \times t_{BA},\\
		r_{32}&=r_3-r_2=c \times t_{CB},
    \end{aligned}
\end{equation}
where $c$ is the speed of light.

Assume that the coordinates of transmitters A, B and C are $ \left(x_A,y_A\right),~ \left(x_B,y_B\right)$ and $ \left(x_C,y_C\right)$, respectively. The coordinate of R, denoted as $\left(x,y\right)$, can be obtained via solving Eq. \eqref{lequ} .
\begin{figure*}[hb] % hb底部，ht为头部
	\centering % 公式居中
	\hrulefill % 添加一条水平线
	\vspace*{8pt} % 调整线与公式之间的距离
\begin{equation}
	\begin{aligned} \label{lequ}
		\left\{
		\begin{array}{lr}
				r_{21}&=\sqrt{\left(x_B-x\right)^2+\left(y_B-y\right)^2}-\sqrt{\left(x_A-x\right)^2+\left(y_A-y\right)^2},\\
				r_{32}&=\sqrt{\left(x_C-x\right)^2+\left(y_C-y\right)^2}-\sqrt{\left(x_B-x\right)^2+\left(y_B-y\right)^2}.
				\end{array}
			\right.
	\end{aligned}	
\end{equation}
%\begin{equation}
%		\begin{aligned}	 \label{lequ2}
%			r_{32}=\sqrt{\left(x_C-x\right)^2+\left(y_C-y\right)^2}-\sqrt{\left(x_B-x\right)^2+\left(y_B-y\right)^2}.
%		\end{aligned}
%%		\end{array}
%%		\right.
%\end{equation}
\end{figure*}
\subsection{Positioning Mean Squared Error (MSE)}\label{MSE Calculation}
The positioning MSE can be approximated as follows. Denote the true receiver location as $\left(x_0,y_0\right)$. Let error vector $\Delta \boldsymbol{u} = \left[\Delta x, \Delta y\right]^T=\left[x-x_0, y-y_0\right]^T$, and $\Delta r_{21}$ and $\Delta r_{32}$ denote the gap between estimated value and actual distance difference
\begin{equation}\label{tba}
	\begin{aligned}
		\Delta r_{21}=\hat{r}_{21}-r_{21}=c\times \Delta t_{BA},
	\end{aligned}
\end{equation}
\begin{equation}\label{tcb}
	\begin{aligned}
		\Delta r_{32}=\hat{r}_{32}-r_{32}=c\times \Delta t_{CB},
	\end{aligned}
\end{equation}
where $\Delta t_{BA}$ denotes the estimation error of $t_{BA}$ and $\Delta t_{CB}$ denotes the estimation error of $t_{CB}$. Distance differences $\Delta r_{21}$ and $\Delta r_{32}$ can be estimated via the first-order partial differential
\begin{equation}
	\begin{aligned}
		\Delta r_{21}=\frac{\partial r_{21}}{\partial x}\big|_{x=x_0} \times \Delta x +\frac{\partial r_{21}}{\partial y}\big|_{y=y_0} \times \Delta y,
	\end{aligned}
\end{equation}
\begin{equation}
	\begin{aligned}
		\Delta r_{32}=\frac{\partial r_{32}}{\partial x}\big|_{x=x_0} \times \Delta x +\frac{\partial r_{32}}{\partial y}\big|_{y=y_0} \times \Delta y,
	\end{aligned}
\end{equation}
where the higher-order terms are ignored.
Thus, we have
\begin{equation}
	\begin{aligned} 
		\begin{bmatrix} \frac{\partial r_{21}}{\partial x}\big|_{x=x_0} & \frac{\partial r_{21}}{\partial y}\big|_{y=y_0} \\ \frac{\partial r_{32}}{\partial x}\big|_{x=x_0} & \frac{\partial r_{32}}{\partial y}\big|_{y=y_0} \end{bmatrix} \begin{bmatrix}
			\Delta x\\
			\Delta y
		\end{bmatrix}=
		\begin{bmatrix}
			c\times \Delta t_{BA}\\
			c\times \Delta t_{CB}
		\end{bmatrix}.
	\end{aligned}
\end{equation}
From Eq. \eqref{lequ}, we have Eq. \eqref{matequ}.
%\end{figure*}
\begin{figure*}[hb] % hb底部，ht为头部
	\centering % 公式居中
	\hrulefill % 添加一条水平线
	\vspace*{8pt} % 调整线与公式之间的距离
\begin{equation}\label{matequ}
	\begin{aligned} 
		\begin{bmatrix} \frac{x_A-x_0}{r_1}-\frac{x_B-x_0}{r_2} & \frac{y_A-y_0}{r_1}-\frac{y_B-y_0}{r_2} \\ \frac{x_B-x_0}{r_2}-\frac{x_C-x_0}{r_3} & \frac{y_B-y_0}{r_2}-\frac{y_C-y_0}{r_3} \end{bmatrix} \begin{bmatrix}
			\Delta x\\
			\Delta y
		\end{bmatrix}=
	\begin{bmatrix}
		c\times \Delta t_{BA}\\
		c\times \Delta t_{CB}
	\end{bmatrix}.
	\end{aligned}
\end{equation}
\end{figure*}

Denote the $2\times2$ matrix in Eq. \eqref{matequ} as $\boldsymbol{G}$ and the vector in the RHS as $\boldsymbol{h}$. When $\boldsymbol{G}$ is full rank, we have $\Delta \boldsymbol{u} = \boldsymbol{G}^{-1}\boldsymbol{h}$. Thus, the positioning MSE matrix is given as follows
\begin{equation}\label{mseforlocation}
	\boldmath{E}\left[\Delta u \Delta u^T\right]=G^{-1}\boldmath{E}\left[hh^T\right]G^{-T},
\end{equation}
where
\begin{equation}\label{mseforlocation2}
	\boldsymbol{h} \boldsymbol{h}^T=\left[\begin{array}{cc}
		\Delta \mathrm{r}_{21}^2 & \Delta \mathrm{r}_{21} \Delta \mathrm{r}_{32} \\
		\Delta \mathrm{r}_{32} \Delta \mathrm{r}_{21} & \Delta \mathrm{r}_{21}^2
	\end{array}\right].
\end{equation}
Letting $\sigma^2_A$, $\sigma^2_B$ and $\sigma^2_C$ denote the estimate MSE of flying time $t_A$,  $t_B$ and $t_C$, respectively, we have
\begin{equation}\label{mseforlocation3}
	\frac{\boldsymbol{E}\left(\boldsymbol{h} \boldsymbol{h}^T\right)}{c^2}=\left[\begin{array}{cc}
		\sigma^2_A+\sigma^2_B & -\sigma^2_B \\
		-\sigma^2_B & \sigma^2_B+\sigma^2_C
	\end{array}\right].
\end{equation}
The positioning error can be expressed as the square root of the trace of MSE matrix as follows
\begin{equation}\label{trace}
	e_p=\sqrt{tr(\boldsymbol{E}\left[\boldsymbol{\Delta u \Delta u^T}\right])}.
\end{equation}


%\vspace{0.3cm}





==> Sec3_SyncProcess.tex <==
%\graphicspath{{figures/Fig_PowerAlloc/}}
%\graphicspath{{figure_yu/FigSync/}}

\section{Theoretical fitting principle for positioning error} \label{Transmittion scheme}
We first investigate the decomposition of estimation error of flying time $t_A$, $t_B$ and $t_C$ into two parts, and analyze each part. 

\subsection{Estimation Error Decomposition for the Flying Time}\label{fly}
The positioning error primarily consists of two parts, one from the atomic clock timing at the transmitter side, and the other from the synchronization error at the receiver side. 

Since it is difficult to achieve perfect alignment of the rising edge from different transmitter-side clocks, the rising edge difference of $10MHz$ square wave multiplied by the speed of light leads to a large distance error. Such error will be characterized in Section \ref{timesec} in detail. Besides, synchronization also leads to estimation error of the correlation peak. An upper bound on the synchronization MSE will be analyzed in Section \ref{syncerror} in detail.

Let $\sigma^2_{clock}$ denote the rising edge error of the atomic clock, and $\sigma^2_{syncA}$, $\sigma^2_{syncB}$ and $\sigma^2_{syncC}$ denote the synchronization error of synchronization signal from transmitter A, transmitter B and transmitter C, respectively. Since the rising edge error of the transmitter clock is independent of the synchronization process, we can approximate $\sigma^2_A=\sigma_{clock}^2+\bar{\sigma}^2_{syncA}$, similarly for $\sigma^2_B$ and $\sigma^2_C$. The positioning error can be obtained from Eq. \eqref{mseforlocation}, Eq. \eqref{mseforlocation2}, Eq. \eqref{mseforlocation3} and Eq. \eqref{trace}.

\subsection{Timing Error of Atomic Clock}\label{timesec}
\begin{figure*}[htpb]
	\centering
	\includegraphics[width=4.5in]{clock.pdf}
	\caption{$\ $Experimental platform of the atomic clock timing error characterization.} \label{clockscene}
	%	\vspace{-0.5cm}%%压缩图片后间隔
\end{figure*}
The transmitters are calibrated by the satellite timing module each second, which is achieved by an atomic clock controlling the time division transmission. The atomic clock timing MSE is denoted as $\sigma_{clock}^2$. To explore its statistical properties, we test the rising edge error of atomic clock. Experimental platform is shown in Fig. \ref{clockscene}. A timing system with an antenna receives the satellite signal, drives the atomic clock to transmit the $10MHz$ square waves, which are then sampled by an oscilloscope. The PPS output of an any wave-form generator (AWG) is adopted as a baseline, whose interval from the next rising edge of $10MHz$ square waves is characterized as the atomic clock delay. Such delay characterizes the systematic error of the rising edge.


\begin{figure}[htpb]
	\centering
	\includegraphics[width=3.0in]{jitter}
	\caption{$\ $Empirical probability distribution of rising edge error of atomic clock.} \label{jitter}
%	\vspace{-0.5cm}%%压缩图片后间隔
\end{figure}
The empirical probability distribution is shown in Fig. \ref{jitter}. The unit of time on the horizontal axis is one second. According to the sampling results, the atomic clock timing error can be considered to be uniformly distributed satisfying $U[0ns,100ns]$.
\subsection{Error of the Synchronization Process}\label{syncerror}
Based on our previous results on the synchronization in \cite{2022arXiv220801559Y}, the synchronization timeline is visualized in Fig. \ref{timeline}.
\begin{figure}[htpb]
	\centering
	\includegraphics[width=3.0in]{TimeIndex}
	\caption{$\ $The timeline of the synchronization.} \label{timeline}
%	\vspace{-0.5cm}%%压缩图片后间隔
\end{figure}
The process of dividing time into chips introduces systematic offsets, denoted as $ \varepsilon $ satisfying uniform distribution $ U(-\frac{T_c}{2},\frac{T_c}{2}) $.

The synchronization process can be divided into three cases. Let estimate ${\hat t}_{Astart}=t_{0,0} $ denote the accurate synchronization estimate as Case 1. In Case 2, the offset lies within a symbol's duration, i.e. ${\hat t}_{Astart}=t_{0,k} $ for certain $ 1\leq \vert k \vert \leq n-1 $, which means that the offset is $k$ chips. In Case 3, consider the offset over a symbol duration, ${\hat t}_{Astart}=t_{2m,k} $ where $  m  \geq 1  $ with $ -n \leq  k  \leq n-1 $ (or $  m  \leq -1  $ with $ -(n-1) \leq  k  \leq n $). The probability of event ${\hat t}_{Astart}=t_{m, k}$ is denoted as $p^A_{m,k}$. The upper bounds on $p^A_{m,k}$ are given by Eq. \eqref{p00}, Eq. \eqref{p0k} and Eq. \eqref{pmk}
\begin{equation}\label{p00}
	{\bar p}^A_{0, 0}=1-{\bar p}^A_{0, 1},
\end{equation}
 \begin{align}\label{p0k}
	p^A_{0, k} \leq {\bar p}^A_{0, k}=\Phi\left(\frac{\frac{\lambda_{s,A}}{2}\left(2\frac{\varepsilon}{T_s}-\frac{k}{n} \right)\left(L-1\right)}{\sqrt{2\frac{k}{n} \left(\frac{\lambda_{s,A}}{2}+\lambda_{b}\right)\left(L-1\right)+\frac{\varepsilon}{T_s}\lambda_{s,A}}}\right).
\end{align}
\begin{figure*}[hb] % hb底部，ht为头部
	\centering % 公式居中
	\hrulefill % 添加一条水平线
	\vspace*{8pt} % 调整线与公式之间的距离
\begin{equation}\label{pmk}
	\begin{aligned}
		p^A_{2m, k} \leq {\bar p}^A_{2m,k}=\Phi\left(\frac{\left(-2m\right)\frac{\lambda_{s,A}}{2}\left[1-2\left(\frac{k}{n}-\frac{\varepsilon}{T_s}\right)\right]-L\frac{\lambda_{s,A}}{2}\left(1-\frac{\varepsilon}{T_s}\right)-\frac{\lambda_{s,A}}{2}\left(2\frac{\varepsilon}{T_s}-\frac{k}{n}\right)}{\sqrt{2\left(\frac{\lambda_{s,A}}{2}+\lambda_{b}\right)\left[\left(L-m\right)-\left(-2m\right)\left(1-2\frac{k}{n}\right)-\frac{k}{n}\right]+\frac{\varepsilon}{T_s}\lambda_{s,A}}}\right).
	\end{aligned}
\end{equation}
\end{figure*}
For estimate ${\hat t}_{Astart}=t_{m,k}$, let $e_{m,k}= t_{m,k} - \varepsilon $ denote the synchronization error. An upper bound on the MSE is denoted as $\bar{\sigma}_{syncA}^2$ in Eq. \eqref{uppbound}, 
\begin{figure*}[hb] % hb底部，ht为头部
	\centering % 公式居中
	\hrulefill % 添加一条水平线
	\vspace*{8pt} % 调整线与公式之间的距离
\begin{align}\label{uppbound}
	\bar{\sigma}_{syncA}^2 \triangleq\int_{-\frac{T_c}{2}}^{\frac{T_c}{2}}\left[e_{0,0}^{2}  \bar{p}^A_{0,0}+2 \sum_{k=1}^{n-1} e_{0, k}^{2}  \bar{p}^A_{0, k}
	+2 \sum_{m=1}^{\infty} \sum_{k=-n}^{(n-1)} e_{2 m, k}^{2}  \bar{p}^A_{2 m, k}\right] p(\varepsilon) d \varepsilon,
\end{align}
\end{figure*}
where $T_c$ is the chip duration, $ p\left(\varepsilon\right)= \frac{1}{T_c}$ for $ \varepsilon \in \left[-\frac{T_c}{2},\frac{T_c}{2}\right] $. We can obtain $\bar{\sigma}_{syncB}^2$ and $\bar{\sigma}_{syncC}^2$ similarly.

%The timing calibration is independent with the synchronization process, so we can approximate that ${\sigma}_A{ }^2=\sigma_{clock}^2+\bar{\sigma}_{syncA}^2$, similar to ${\sigma}_B{ }^2$ and ${\sigma}_C{ }^2$. Then plug them in the formula Eq. \eqref{mseforlocation}, Eq. \eqref{mseforlocation2} and Eq. \eqref{mseforlocation3} to calculate the MSE of positioning.

%\subsection{Code Division Transmission}\label{Code Division Transmission}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 
%A, B and C send various synchronization sequences at the same time. The transmitters are calibrated by the timing module every second. MSE of calibration is denoted as $\sigma_{sec}^2$. To A's synchronization, signals from B and C cause distraction. Nevertheless, each transmitter can send longer sequence in the same duration than time division transmission, which benefits increase of synchronization accuracy. Thus, the trade-off makes it necessary to compare the two transmission schemes.
%
%The synchronization process for code division transmission is similar to that for time division transmission. Let $\{s_{Ai}:1\leq i \leq L_2\}$ denote A's synchronization sequence.
%\begin{equation}
%	\begin{aligned} \label{equ.auto-correlation2}
%		{\hat t}_{Astart}&=\arg \max _{t_{Astart}}\left\{\sum_{i=1}^{L}\left\{u_{i}^{t_{Astart}} \times\left(2 s_{Ai}-1\right)\right\}\right\},\\
%	\end{aligned}
%\end{equation}
%It is worth noting that $u_{i}^{t_{Astart}}$ in Eq. \eqref{equ.auto-correlation2} here contains not only photons of the target signal and noise photons, but also photons of the interfering signals from other two transmitters. The derivation of $\bar{\sigma}_{sync}^2$ is similar to that in Section. \ref{Time Division Transmission}. But we need to introduce $\Lambda_i$ as the intensity of interference signals. With the same time overhead, the sequence length $L$ can be increased to $L_2$. Therefore, The upper bounds on $p_{m,k}$ is given by
%\begin{equation}
%	{\bar p}_{0, 0}=1-{\bar p}_{0, 1}.
%\end{equation}
%\begin{align}\label{case2}
%	p_{0, k} \leq {\bar p}_{0, k}=\Phi\left(\frac{\frac{\lambda_{s}}{2}\left(2\varepsilon-\frac{k}{n}\right)\left[L_2-1\right]}{\sqrt{2\frac{k}{n}\left(\frac{\lambda_{s}}{2}+\lambda_{b}+\Lambda_i\right)\left[L_2-1\right]+\varepsilon\lambda_{s}}}\right).
%\end{align}
%\begin{equation}
%	\begin{aligned}\label{case3}
%		p_{2m, k} \leq {\bar p}_{2m,k}=\Phi\left(\frac{\left(-2m\right)\frac{\lambda_{s}}{2}\left[1-2\left(\frac{k}{n}-\varepsilon\right)\right]-L_2\frac{\lambda_{s}}{2}\left[1-\varepsilon\right]-\frac{\lambda_{s}}{2}\left(2\varepsilon-\frac{k}{n}\right)}{\sqrt{2\left(\frac{\lambda_{s}}{2}+\lambda_{b}+\Lambda_i\right)\left[\left(L_2-m\right)-\left(-2m\right)\left(1-2\frac{k}{n}\right)-\frac{k}{n}\right]+\varepsilon\lambda_{s}}}\right).
%	\end{aligned}
%\end{equation}
%
%Ideally, $\bar{\sigma}_{sync}$ can be calculated as the same as Eq. \eqref{uppbound}. And we can approximate that ${\sigma}_A{ }^2=\sigma_{sec}^2+\bar{\sigma}_{syncA}^2$, similar to ${\sigma}_B{ }^2$ and ${\sigma}_C{ }^2$, which can lead to the MSE of location in Eq. \eqref{mseforlocation} with Eq. \eqref{mseforlocation3}. However, $\Lambda_i$ is difficult to display or calculated explicitly in equations, so as MSE of location. Consequently, Section. \ref{Theoretical fitting and simulation verification} only demonstrates theoritical fitted value for MSE of location in time Division transmission scheme. 
%
%Besides, directly calculating the correlation value of multichannel signals makes the accuracy of synchronization poor. Especially when the receiver is close to a certain transmitter, the signal intensity of the transmitter is too large, which seriously affects the synchronization of other signals. Therefore, it is necessary to introduce an interference elimination algorithm Algorithm. \ref{IEA algo} to reduce $\Lambda_i$ as much as possible. The strongest interference mainly comes from the signal of the closest transmitter, taking A for example, with the highest intensity. The synchronization signal itself suffers relatively little interference and therefore has relatively best synchronization accuracy in State. \ref{sync1} of Algorithm. \ref{IEA algo}. Based on ${\hat t}_{Astart}$ and the signal intensity, the signal from transmitter A is simulated according to the uniform distribution, which is the conditional distribution of the Poisson distribution for a given parameter. After cancelling the simulated interference of transmitter A above, the signals from B and C are synchronized to get new ${\hat t}_{Bstart}$ and ${\hat t}_{Cstart}$. Repeat the above procedure for the second strongest signal (assuming that it is from transmitter B), and update ${\hat t}_{Cstart}$. After interference elimination, the target is to get more accurate ${\hat t}_{Astart}$, ${\hat t}_{Bstart}$ and ${\hat t}_{Cstart}$.
%
%\begin{algorithm}[htb]
%	\caption{ Interference elimination algorithm for code division transmission's synchronization.}
%	\label{IEA algo}
%	\begin{algorithmic}[1]
%		\Require
%		
%		Three synchronization sequences, $\{s_{Ai}:1\leq i \leq L_2\}$, $\{s_{Bi}:1\leq i \leq L_2\}$ and $\{s_{Ci}:1\leq i \leq L_2\}$;
%		
%		The set of start chip index, $\{t_{Astart}\}  $, $\{t_{Bstart}\}  $ and $\{t_{Cstart}\}  $;
%		
%		The vector of pulse number correlated with sequences based on start chip index $ t_{Astart} $, $\boldsymbol{u}^{t_{Astart}}$, $\boldsymbol{u}^{t_{Bstart}}$ and $\boldsymbol{u}^{t_{Cstart}}$;
%		
%		\Ensure
%		Arriving time of synchronization sequences from three transmitters, ${\hat t}_{Astart}$, ${\hat t}_{Bstart}$ and ${\hat t}_{Cstart}$;
%		\State Figure up ${\hat t}_{Astart}$ by Eq. \eqref{equ.auto-correlation2} with maximum value $Cormax_A$, so as ${\hat t}_{Bstart}$ and ${\hat t}_{Cstart}$, assuming $max\{Cormax_B , Cormax_C\} \leq Cormax_A$;
%		\label{sync1}
%%		 ${\hat {\lambda}_{As}}=\frac{2\times Cormax_A}{L_2}$,
%		\State Put $\hat {\lambda}_{As}$ photons uniformly in symbol 1 's duration with ${\hat t}_{Astart}$ as the start of Arriving time of A's synchronization sequence. These photons are called A's analog photons; According to the set of start chip index and symbol duration, A's analog photons can be divided into elements in vector $\boldsymbol{v}_A^{t_{Bstart}}$ and $\boldsymbol{v}_A^{t_{Cstart}}$;
%		\label{code:fram:trainbase}
%		\State \begin{equation}
%			\begin{aligned} \label{equ.auto-correlation3}
%				{\hat t}_{Bstart}&=\arg \max _{t_{Bstart}}\left\{\sum_{i=1}^{L}\left\{\left(u_{i}^{t_{Bstart}}-{v_A}_{i}^{t_{Bstart}}\right) \times\left(2 s_{Bi}-1\right)\right\}\right\},\\
%			\end{aligned}
%			\end{equation}
%		with maximum value $Cormax_B$.
%		\begin{equation}
%		\begin{aligned} \label{equ.auto-correlation4}
%			{\hat t}_{Cstart}&=\arg \max _{t_{Cstart}}\left\{\sum_{i=1}^{L}\left\{\left(u_{i}^{t_{Cstart}}-{v_A}_{i}^{t_{Cstart}}\right) \times\left(2 s_{Ci}-1\right)\right\}\right\},\\
%		\end{aligned}
%		\end{equation}
%	with maximum value $Cormax_C$, assuming $Cormax_C \leq Cormax_B$. 
%%	${\hat {\lambda}_{Bs}}=\frac{2\times Cormax_B}{L_2}$,
%		\label{code:fram:add}
%		\State Put $\hat {\lambda}_{Bs}$ photons uniformly in symbol 1 's duration with ${\hat t}_{Bstart}$ as the start of Arriving time of B's synchronization sequence. These photons are called B's analog photons; According to the set of start chip index and symbol duration, B's analog photons can be divided into elements in vector $\boldsymbol{v}_B^{t_{Cstart}}$;
%		\label{code:fram:classify}
%		\State\begin{equation}
%			\begin{aligned} \label{equ.auto-correlation5}
%				{\hat t}_{Cstart}&=\arg \max _{t_{Cstart}}\left\{\sum_{i=1}^{L}\left\{\left(u_{i}^{t_{Cstart}}-{v_A}_{i}^{t_{Cstart}}-{v_B}_{i}^{t_{Cstart}}\right) \times\left(2 s_{Ci}-1\right)\right\}\right\},\\
%			\end{aligned}
%		\end{equation}
%		\label{code:fram:select} \\
%		\Return ${\hat t}_{Astart}$, ${\hat t}_{Bstart}$ and ${\hat t}_{Cstart}$;
%	\end{algorithmic}
%\end{algorithm}


















==> Sec4_Constellation.tex <==
%\graphicspath{{figure_yu/FigSimu/}}

\section{Simulation verification for positioning error}  \label{Theoretical fitting and simulation verification}
We conduct simulation to show the accuracy of theoretical error as shown in Section \ref{fly}. Lay the three transmitters as shown in Fig. \ref{LocationRange}, and locate receiver R in the range represented by the purple box.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{LocationRange.pdf}
	\caption{$\ $Schematic diagram of location range.} \label{LocationRange}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure}

%\subsection{Time Division Transmission}\label{Time Division Transmission4}
Assume that transmitters A, B and C send the same synchronization sequence with length $L=256$ in a time-division manner with duration $T=300us$. Assume that the transmission symbol rate is $ 1Mbps$. The transmission power is $100mW$ and the detector receiving area is $1.77\times10^{-4}~m^2$. The transmitter divergence angle is $120^\circ$. Set $ \lambda_{b}=1$ as the noise intensity. After calculating the link gain for line of sight (LOS) UV communication and signal intensity $\lambda_{s}$, we can obtain the approximate upper bound on the average positioning error for each receiver position as well as the correspounding simulation results. The average error is $\sqrt{MSE}$. The sampling rate at the receiver is set to $100MHz$ due to UV PMT dead time of approximately $10$ ns. As $ \lambda_{b}$ is relatively small, we apply a cut-off function for signal intensity $\lambda_{s}$, which is clipped to $100$ if exceeding $100$.
%\begin{equation}\label{cutoff}
%	\begin{aligned} 
%	\lambda_{s}=	\left\{
%		\begin{array}{lr}
%			\lambda_{s},&~~~\lambda_{s}\leq 100;\\
%			100,&~~~\lambda_{s}\textgreater  100.
%		\end{array}
%		\right.
%	\end{aligned}
%\end{equation}

\subsection{Ideal Case: Perfectly Synchronized Transmitters}\label{ssec.ideal}
We first discuss an ideal case where complete clock synchronization is achieved among the three transmitters  with $\sigma_{clock}=0 $. Fig. \ref{d_std_pic_secErr0_calcu} shows the theoretical average positioning error in Eq. \eqref{trace}.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_pic_secErr0_calcu}
	\caption{$\ $Theoretical average positioning error with $\sigma_{clock}=0 $.} \label{d_std_pic_secErr0_calcu}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure}
In the simulation with $\sigma_{clock}=0 $, the simulated positioning error is shown in Fig. \ref{d_std_pic_secErr0}, which is in good agreement with the theoretical error in Fig. \ref{d_std_pic_secErr0_calcu}. Lower positioning error can be observed in the center of location range.
\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_pic_secErr0}
	\caption{$\ $Simulated average positioning error with $\sigma_{clock}=0 $.} \label{d_std_pic_secErr0}
	    	\vspace{-0.3cm}%%压缩图片后间隔
\end{figure}

In order to explore the effect of transmission power on the positioning error, we carry out more simulations and compare the results with the theoretical one, as shown in Fig. \ref{d_std_mean_pi}. The horizontal axis represents the transmission power and vertical axis represents the average positioning error of $81$ receiver points in the location range in Fig. \ref{LocationRange}. It can be found that the positioning accuracy can be improved as the transmission power increases. However, as the transmission power increases to a certain extent, the accuracy improvement becomes saturated. This is due to the limitation of the PMT's sampling rate at the receiver, where the synchronization accuracy and positioning accuracy cannot be further improved via increasing the transmission power.
\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_mean_pi}
	\caption{$\ $Theoretical and simulation results on the average positioning error with $\sigma_{clock}=0 $.} \label{d_std_mean_pi}
   	\vspace{-0.3cm}%%压缩图片后间隔
\end{figure}
\subsection{Actual Case: Non-negligible Timing Error at Different Transmitters}
In the actual positioning system realization, a challenge is to consider the synchronization bias between different transmitters. After receiving the satellite PPS (pulse per second) signal at each transmitter, a square wave rising edge with a frequency of $10MHz$ is adopted to control the transmission of the synchronous sequence. The error of $10MHz$ square wave superimposed by the error of 1 PPS signal can be considered to meet the uniform distribution $U[0ns,100ns]$ according to Section \ref{timesec}.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_pic_secErr50_calcu}
	\caption{$\ $Theoretical average positioning error with non-negligible rising-edge bias.} \label{d_std_pic_secErr50_calcu}
    	\vspace{-0.3cm}%%压缩图片后间隔
\end{figure}

In the simulation with timing bias between different transmitters, we assume a uniformly distributed random variable satisfying $U[0ns,100ns]$ on sending time difference of each transmitter under hardware realization. The positioning range is consistent with that in Subsection \ref{ssec.ideal}. Both theoretical and simulation results show that the transmitter-side timing error has a significant impact on the positioning accuracy. Note that there exists a triangle with three transmitters as the vertices. Inside the triangle, the simulated positioning error shows agreement with the theoretical one, all around $10$ meters. Outside the triangle, the positioning accuracy and the agreement between the theoretical accuracy and simulated one becomes degraded, primarily due to the accuracy of the first-order approximation in the theoretical derivation.
\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_pic_secErr50}
	\caption{$\ $Simulated average positioning error with non-negligible rising-edge bias.} \label{d_std_pic_secErr50}
%    	\vspace{-0.3cm}%%压缩图片后间隔
\end{figure}
\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_mean_pivary}
	\caption{$\ $Theoretical and simulated average positioning error under transmitter timing error.} \label{d_std_mean_pi50}
    	\vspace{-0.3cm}%%压缩图片后间隔
\end{figure}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{d_std_mean_pivary2_2}
	\caption{$\ $Theoretical and simulated average positioning error inside the triangle under transmitter timing error.} \label{d_std_mean_pi2}
    	\vspace{-0.3cm}%%压缩图片后间隔
\end{figure}

In order to explore the influence of transmission power on the positioning accuracy with timing bias, we also conduct more simulations and compare the results with the theoretical ones, as shown in Fig. \ref{d_std_mean_pi50}. Both theoretical and simulated values are obtained assuming uniform distribution of misalignment in the transmitter clock rising edge under different parameters.

Similarly, the positioning error decreases with the transmission power. However, when the transmission power increases to a certain extent, the positioning error reduction becomes saturated. This is not only due to the limitation of the PMT's sampling rate at the receiver but also due to the atomic clock error satisfying uniform distribution at the transmitters, where the latter is the main reason of the positioning accuracy degradation compared with those shown in Fig. \ref{d_std_mean_pi} in Section \ref{ssec.ideal}. In the simulation where the rising edge error satisfies $U[0ns,100ns]$, the points in the region outside the triangle shows bigger gap between the simulated average positioning error and the theoretical one. When the positioning range is inside the triangle as shown in Fig. \ref{d_std_mean_pi2}, the gap decreases significantly. Through the comparison of theoretical and simulated results, a larger rising edge misalignment of the transmitter clock leads to a larger positioning error. Such results imply that the positioning accuracy can be improved via more accurate clock alignment.


%\subsection{Code Division Transmission}\label{Code Division Transmission4}                         
%%A, B and C send synchronization sequences at the same time. $\Lambda_i$ is half of the sum of other transmitters' signal intensity in Eq. \eqref{case2} and Eq. \eqref{case3}. Other parameters are set the same as Section \ref{Time Division Transmission4}.
%%                         
%%Fig. \ref{d_std_pic_cd} shows the theoretical fitted value on location MSE in Eq. \eqref{mseforlocation} with Eq. \eqref{mseforlocation3} calculated following derivation in Section \ref{Code Division Transmission}. There are some outliers with large values near a transmitter. 
%%\begin{figure}[htbp]
%%	\centering
%%	\includegraphics[width=5.8in]{d_std_pic_cd}
%%	\caption{$\ $Theoretical fitted value on location MSE in code division transmission.} \label{d_std_pic_cd}
%%	%    	\vspace{-1.0cm}%%压缩图片后间隔
%%\end{figure}
%For code division transmission scheme, the uncertain interference is hard to quantify. Thus, we utilize the simulation results with interference elimination algorithm Algorithm. \ref{IEA algo} to characterize the localization accuracy. A, B and C send various synchronization sequences, which length satisfies $L=256\times 3$ to equalize the valid time overhead, at the same time. In simulation, other parameters are consistent with Section. \ref{Time Division Transmission4}. Similarly, the location accuracy is relatively better in the center of location range with favourable geometric topology. Nevertheless, there are outliers with large location error. Some outliers near transmitter A are due to the signal intensity of A being too strong, which seriously interferes with the synchronization of transmitter B and transmitter C. The outliers in the upper left and upper right corner are due to they don't lay in the triangle formed by the lines between one transmitter and another. Because of this geometry, the location accuracy is significantly reduced when the synchronization accuracy is slightly reduced due to interference.
%
%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=5.5in]{d_std_pic_simu_cd_remove}
%	\caption{$\ $Simulation results on location average error in code division transmission.} \label{d_std_pic_simu_cd}
%	%    	\vspace{-1.0cm}%%压缩图片后间隔
%\end{figure}

==> Sec5to6_ConcluAckn.tex <==
%\graphicspath{{figure_yu/FigExp/}}



\section{Outdoor Positioning Experiment} \label{Outdoor Location Experiment}
%In outdoor experiments, we execute the time division transmission that A, B and C send synchronization sequences, which length satisfies $L=256$, in turn at fixed time interval $T=300us$. The symbol rate of transmission is $ 1Mbps$.
%%\begin{figure}[htbp]
%%	\centering
%%	\includegraphics[width=5.5in]{expLoc}
%%	\caption{$\ $Schematic diagram of location in outdoor experiment.} \label{expLoc}
%%	%    	\vspace{-1.0cm}%%压缩图片后间隔
%%\end{figure}
%The outdoor real-time experiment was carried out two times in total. Lay the three transmitters and the receiver R as Fig. \ref{TDOA} shows and the process of the outdoor experiment follows Fig. \ref{expPro}. R is placed in the triangle formed by the lines between one transmitter and another. 

\subsection{Hardware Realization of the Positioning System}
The system block diagram and experimental system hardware realization are shown in Fig. \ref{expPro} and Fig. \ref{hardBlo}, respectively.

\begin{figure*}[htbp]
	\centering
	\includegraphics[width=4.5in]{expPro4.pdf}
	\caption{$\ $The functional block diagram of UV communication system.} \label{expPro}
	\vspace{-0.2cm}%%压缩图片后间隔
\end{figure*}

\begin{figure*}
	\centering
	\includegraphics[width=4.5in]{tran_uti.pdf}
	\caption{The resource utilization after hardware implementation at the transmitter side.}
	\label{utiTran}
	\vspace{-0.2cm}%%压缩图片后间隔
\end{figure*}

\begin{figure*}
	\centering
	\includegraphics[width=4.5in]{recei_uti.pdf}
	\caption{The resource utilization after hardware implementation at the receiver side.}
	\label{uti}
	\vspace{-0.2cm}%%压缩图片后间隔
\end{figure*}

\begin{figure*}[htbp]
	\centering
	\includegraphics[width=4.5in]{hardwareBlocks.pdf}
	\caption{$\ $The hardware realization blocks for the UV positioning system.} \label{hardBlo}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure*}

At the transmitter side, the timing system including an antenna (unicorecomm, UT4B0) send Pulse Per Second (PPS) to Field Programmable Gate Array (FPGA) to control the time-division transmission by the atomic clock (CHENGDU ELECSPN, XHTF1033$\_$CPT), whose timing error satisfies uniform distribution $U[0ns,100ns]$ according to Section \ref{timesec}. The UV LED (266nm) transmits ultraviolet pilot signal modulated by FPGA. The resource utilization after hardware implementation at the transmitter side is shown in Fig. \ref{utiTran}.

 At the receiver side, PMTs are employed as the photon-detector, which can convert the received
 photoelectrons to analog pulses such that photon counting can be realized via pulse counting. 
 HAMAMATSU PMT (R7154 module) detector is sealed into a shielding box, which is integrated
 with an UV optical filter that passes the light signal of wavelength around 266 nm and blocks
 the solar background radiation on other wavelengths. Analog-to-digital converters (ADCs) are employed such that the rising edge detection can be performed in the digital domain. The digital signal processing of synchronization and computation of the arrival time differences between receiving signals from different transmitters are performed sequentially on the FPGA board. The resource utilization after hardware implementation at the receiver side is shown in Fig. \ref{uti}. Then, the arrival time differences are sent to the receiver-side personal computer (RX-PC) through serial ports to obtain the real-time positioning results according to Eq. \eqref{lequ}. 
 
 The corresponding real-time hardware realization is shown in Fig. \ref{hardBlo}. An atomic clock including an antenna is welded in the FPGA board and the timing system is connected to the FPGA board through pin interfaces. The UV LED consists of an array of $3\times3$ UV light beads. The spectral response of PMT ranges from $160nm$ to $320nm$ and the detection bandwith is wider than $200MHz$. The ADC sampling line connects the PMT to the ADC on the FPGA board, which outputs the processed data to the PC terminal.

We carried out a preliminary test including twelve receiver points on a small lawn, which is denoted as Experiment $\Rmnum{1}$ as shown in Table \ref{table.outdoor1}. The specific position coordinates and error results are presented. Points A, B and C indicate three transmitters, whose coordinates are shown in Table \ref{table.outdoor1}. Three transmitters A, B and C send synchronization sequences in a time-division manner with length $L=256$ and fixed time interval $T=300us$. The symbol rate of transmission is $ 1Mbps$ and the transmission power is $150mW$. The positioning error for a receiver point is calculated as the average error in ten estimates based on measurements. Theoretical error denotes the corresponding theoretical positioning error. The experimental average positioning error over the twelve points is $10.2130m$, while the corresponding theoretical average positioning error is $11.1303m$.

\subsection{Outdoor Test on the Playground}\label{testp}

%
%Weather: Sunny
%
%Air temperature: $\qty{25}{\degreeCelsius} \sim \qty{34}{\degreeCelsius}$
%
%Air Quality Index (AQI): $27$

We conducted an outdoor experiment in the university playground. The test was completed on July 23, 2023. The weather was sunny, with temperatures ranging from 25$^{\circ}$C to 34$^{\circ}$C, and the air quality index (AQI) was 27. The hardware and experimental processing are the same as those in the preliminary test. The transmission power is $150mW$.
\begin{figure}[htbp]
	\centering
	\includegraphics[width=3.0in]{playground.pdf}
	\caption{$\ $The positions of three transmitters and receiver $R$ in the outdoor experiment on the university playground.} \label{playground}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure}
%The outdoor real-time experiment was carried out two times in total. 
Lay the three transmitters and the receiver R as shown in Fig. \ref{playground}. The hardware processing of outdoor experiment follows Fig. \ref{expPro}. R is placed in the triangle connected by the three transmitters.

The positioning results are shown in Fig. \ref{positionRst}, where the three transmitters are marked as three big blue circles at three known locations. Each solid colored dot denotes the real receiver position, and the asterisk mark of the corresponding color denotes the positioning estimate of the receiver. The positioning performances at nine positions are tested, where ten estimates are obtained for each positioning. Clustering effect of the estimated position can be observed with small internal variance. The average distance from the ten estimated values to the center of the ten positions can reach the level around $2.1159m$. This is due to the fact that the positioning error mainly comes from the misalignment in the rising edge of the transmitter clock in the short time duration.
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=4.2in]{zuobiaotu3}
	\caption{$\ $The positioning results in the outdoor experiment on the university playground.} \label{positionRst}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure*}

As shown in Table. \ref{table.outdoor1}, Experiment $\Rmnum{2}$ denotes the outdoor test including nine receiver points in total on the playground. The experimental average positioning error over the all nine points is $11.2000m$, while the corresponding theoretical average positioning error is $10.6725m$.
\subsection{Outdoor Test on a Grand Lawn}

%Date: 10/26/2023
%
%Weather: Cloudy
%
%Air temperature: $\qty{14}{\degreeCelsius} \sim \qty{28}{\degreeCelsius}$
%
%Air Quality Index (AQI): $90$

\begin{figure*}[htbp]
	\centering
	\includegraphics[width=4.5in]{lawn.pdf}
	\caption{$\ $The positions of three transmitters and receiver $R$ in the outdoor experiment on the larger grand lawn.} \label{lawn}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure*}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=4.2in]{zuobiaotu4}
	\caption{$\ $The positioning results in the outdoor experiment on the grand lawn.} \label{positionRst2}
%   	\vspace{-0.5cm}%%压缩图片后间隔
\end{figure*}

We further conducted another outdoor test on a larger grand lawn on Hefei Binhu Anshang Grassland, where the layout of three transmitters and receiver R is shown in Fig. \ref{lawn}. The test was completed on October 26, 2023. The weather was cloudy, with temperatures ranging from 14$^{\circ}$C to 28$^{\circ}$C, and the air quality index (AQI) was 90. Receiver R is placed in the triangle connected by the three transmitters. The positioning at seventeen positions are tested, where ten estimates are obtained for each positioning. The hardware and experimental processing are the same as those in Section \ref{testp}. The transmission power is adjusted to $1W$.

The positioning results are shown in Fig. \ref{positionRst2}. The clustering effect of the estimated position near the actual position can also be observed. However, compared with Fig. \ref{positionRst}, the internal variance of the cluster is larger. We compute the average distance from the ten estimated values to the center of mass of the estimated cluster, where the average over seventeen receiver points reaches $5.0780m$. At some points, two clusters can be observed. This is due to wider distribution of the three transmitters, which tends to cause variations of misalignment. 

As shown in Table \ref{table.outdoor1}, the experimental average positioning error over the seventeen points in Experiment $\Rmnum{3}$ is $9.8310m$, while the corresponding theoretical average positioning error is $11.4894m$. Such results validate the consistency of outdoor experiments with the theoretical average positioning error. 

\begin{table*}[h]
	\begin{center}
		\renewcommand\arraystretch{2}
		\captionof{table}{The positioning accuracy in the three scenarios of outdoor experiments (unit m).}
		\label{table.outdoor1}
		\begin{tabular}{| c | c | c | c | c | c | c |}
			\hline
			Index &  $A$ & $B$ & $C$   & Experimental Error & Theoretical Error \\ \hline
			
			
			$\Rmnum{1}$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			$ 10.2130 $& $ 11.1303 $     \\ \hline
			
			$\Rmnum{2}$ &$\left(0,0\right)$ & $\left(75.6,0\right)$ & $\left(32.2,76.6\right)$ 
			& $ 11.2000 $ & $ 10.6725 $ \\ \hline
			
			$\Rmnum{3}$ &$\left(0,0\right)$ & $\left(128.6,122.8\right)$& $\left(247.1,0\right)$ & 
			$ 9.8310 $& $ 11.4894 $     \\ \hline
			%			$\Rmnum{1}-2$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(21.7153,3.5276\right) $ & $ 11.6755 $ & $ 11.5944 $  \\ \hline
			%			
			%			$\Rmnum{1}-3$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(17.4895,20.4384\right) $ & $ 15.1600 $ & $ 10.8476 $   \\ \hline
			%			
			%			$\Rmnum{1}-4$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(24.7577,42.8638\right) $ & $ 5.7075 $  & $ 11.6780 $  \\ \hline
			%			
			%			$\Rmnum{1}-5$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(60.6912,30.2228\right) $ & $ 4.0647 $  & $ 12.7806 $ \\ \hline
			%			
			%			$\Rmnum{1}-6$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(44.7037,26.9522\right) $ & $ 6.3853 $ & $ 10.4406 $  \\ \hline
			%			
			%			$\Rmnum{1}-7$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(44.7333,33.0195\right) $ & $ 3.6853 $  & $ 10.7720 $   \\ \hline
			%			
			%			$\Rmnum{1}-8$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(36.6790,32.4907\right) $ & $ 10.4699 $ & $ 10.3891 $    \\ \hline
			%			
			%			$\Rmnum{1}-9$ &$\left(0,0\right)$ & $\left(75.6,0\right)$& $\left(32.2,76.6\right)$ & 
			%			$ \left(36.8159,27.0755\right) $ & $ 3.3579 $ & $ 10.1524 $    \\ \hline
			%			
			%			$\Rmnum{2}-1$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(29.1830,22.4678\right) $ & $ 16.2033 $& $ 10.1721 $     \\ \hline
			%			
			%			$\Rmnum{2}-2$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(33.0000,0\right) $ & $ 18.1455 $ & $ 12.3279 $    \\ \hline
			%			
			%			$\Rmnum{2}-3$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(32.0000,6.0000\right) $ & $ 3.2542 $ & $ 10.9204 $    \\ \hline
			%			
			%			$\Rmnum{2}-4$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(38.4947,21.5577\right) $ & $ 11.0701 $ & $ 10.5475 $    \\ \hline
			%			
			%			$\Rmnum{2}-5$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(29.3599,19.4026\right) $ & $ 7.2754 $ & $ 10.0984 $    \\ \hline
			%			
			%			$\Rmnum{2}-6$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(36.1509,21.6734\right) $ & $ 9.3138 $ & $ 10.3465 $    \\ \hline
			%			
			%			$\Rmnum{2}-7$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(36.5379,18.6887\right) $ & $ 14.0890 $ & $ 10.2660 $    \\ \hline
			%			
			%			$\Rmnum{2}-8$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(34.4259,16.3473\right) $ & $ 6.6767 $ & $ 10.1378$    \\ \hline
			%			
			%			$\Rmnum{2}-9$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(32.5232,22.0620\right) $ & $ 10.2533 $ & $ 10.1796 $    \\ \hline
			%			
			%			$\Rmnum{2}-10$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(41.2765,20.2358\right) $ & $ 12.2475 $ & $ 10.8005 $    \\ \hline
			%			
			%			$\Rmnum{2}-11$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(41.5534,17.4534\right) $ & $ 11.6607 $ & $ 10.6980 $    \\ \hline
			%			
			%			$ \Rmnum{2}-12$ &$\left(30.2,53.9\right)$ & $\left(0,0\right)$& $\left(60.7,0\right)$ & 
			%			$ \left(36.0000,3.0000\right) $ & $ 13.7998 $ & $ 11.5748 $    \\ \hline
		\end{tabular}
		%		\vspace{-3em} 
	\end{center}
\end{table*}

\subsection{Further Accuracy Improvement Roadmap}
%The specific position coordinates and error results are presented in Table. \ref{table.outdoor1}. A, B and C indicate three transmitters. The table shows their coordinates. Location error for a receiver point is the average of the errors in the ten estimates during the short time for positioning measurements. Theoretical error is the corresponding fitting result. Experiment $\Rmnum{2}$ denotes the outdoor test including nine receiver points in total on the playground. The average positioning error of the all nine points in experiment $\Rmnum{2}$ is $11.2000m$, while the corresponding theoretical fit average is $10.6725m$. Experiment $\Rmnum{3}$ including seventeen receiver points is carried out on a grand lawn as Fig. \ref{lawn} shows. Similarly, the average positioning error of the seventeen points in experiment $\Rmnum{3}$ is $9.8310m$, while the corresponding theoretical fit average is $11.4894m$. The numerical consistency indicates that the results of outdoor experiments verify the accuracy of the theoretical fitting values. It is worth noting that when the error in the rising edge of the transmitter clock is reduced, the positioning accuracy will be significantly improved.



In addition to changing the transmitter-side atomic clock with that with smaller error in the rising edge, the positioning performance can also be improved via time synchronization processing between the three transmitters. We simulate a virtual differential positioning, where the timing error estimate is randomly selected from all ten estimates for each receiver point to obtain A-B clock correction and B-C clock correction. After the correction, the average positioning error over all nine points in Experiment $\Rmnum{2}$ can reach $3.1269m$; and the average positioning error over seventeen points in Experiment $\Rmnum{3}$ can reach $7.4675m$. This is due to the observation that in Experiment III, the $10$ estimates are sometimes divided into more than one cluster, such that the positioning error reduction is smaller than that of Experiment $\Rmnum{2}$. Such results imply that if the clock system misalignment can be estimated and transmitted to the receiver, the positioning accuracy can potentially be significantly improved. 




%The location error is $2.9867m$, while its corresponding theoretical fitted error is $ 2.3277m $ and simulation error is $2.4512m $. Consistency among the three error results shows the reliability of time division transimission scheme in hardware implementation and practical application. 

%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=5.5in]{exp_err_rst}
%	\caption{$\ $Results of positioning error in outdoor experiments.} \label{expErr}
%	%    	\vspace{-1.0cm}%%压缩图片后间隔
%\end{figure}



%\begin{table*}[h]
%	\begin{center}
%		\renewcommand\arraystretch{2}
%		\captionof{table}{The location results for outdoor experiment.}
%		\label{table.outdoor1}
%		\begin{tabular}{| c | c | c | c | c | c | c |}
%			\hline
%			$r_{13}$ &$\hat{r}_{13}$ & $r_{23}$ & $\hat{r}_{23}$  & $ R $ & $ \hat{R} $  & Location error \\ \hline
%		$-7.6m$ &$-12m$ & $2.98m$& $0m$ & $ \left(32.12m,13.32m\right) $ & $ \left(33.7200m,15.8419m\right) $  & $ 2.9867m$ \\ 
%			\hline
%		\end{tabular}
%%		\vspace{-3em} 
%	\end{center}
%\end{table*}

==> Sec6_SeqOptimization.tex <==
\graphicspath{{figure_yu/FigModel/}}

\section{Three-dimensional Space Positioning Design} \label{Three-dimensional space positioning design}
Three-dimensional positioning requires more information than two-dimensional positioning, which are position coordinates and time differences of at least four transmitters. For the 3D location network we design, the transmitters are arranged in pairwise equidistant form as Fig. \ref{Loc3D} shows. The distance between each transmitter is $100m$. All the transmitters marked with blue points form a UV positioning network.
 \begin{figure}[htbp]
	\centering
	\includegraphics[width=5.5in]{Loc3D}
	\caption{$\ $Schematic diagram of TDOA principle.} \label{Loc3D}
	%    	\vspace{-1.0cm}%%压缩图片后间隔
\end{figure}

First, we need to find the approximate range of the receiver, then we carry out accurate positioning within that range. As the receiver is in the cube surrounded by a purple border, we can find that approximate range by part of the vertices of the cube. Although only four vertices of the cube are needed as the transmitters to locate the receiver, there is a high probability that the receiver is not inside the tetrahedron or even plane formed by these four points. Such geometric characteristics will greatly reduce the location accuracy. Therefore, we decided to use six transmitters to locate the receiver. Taking Fig. \ref{Loc3D} as an example, three transmitters are chosen from the plane $Z=100m$ and other three transmitters are chosen from the plane $Z=0m$ to locate the receiver inside the pentahedron made up of these six points. These transmitters are marked with green circles. 

\begin{algorithm}[htb]
	\caption{ Algorithm for three-dimensional space positioning.}
	\label{3D algo}
	\begin{algorithmic}[1]
		\Require
		
		Each transmitters' own synchronization sequence;
		
		
		
		\Ensure
		Arriving time of synchronization sequences from six transmitters;
		\State All transmitters in plane $Z=100m$ transmitt their synchronization sequences at the same time in the code division transmission scheme. And the receiver figure out all correlation peak values $Cormax$ for every synchronization sequence. Among them, $Cormax_A$, $Cormax_B$ and $Cormax_C$ are the three largest values. So transmitters $A$, $B$ and $C$ are chosen for accurate positioning;
		\label{3D1}
		%		 ${\hat {\lambda}_{As}}=\frac{2\times Cormax_A}{L_2}$,
		\State All transmitters in plane $Z=0m$ are handled as the same as State. \ref{3D1} and transmitters $E$, $F$ and $G$ are chosen for accurate positioning;
		\label{3D2}
		\State The six selected transmitters transmitt their synchronization sequences in turn at fixed time interval $T$ according to the time division transmission scheme. And the receiver figure out arriving time of signals from six transmitters;
		\label{3D3}\\
		\Return Arriving time of synchronization sequences from six transmitters;
	\end{algorithmic}
\end{algorithm}

Algorithm. \ref{3D algo} shows the algorithm for three-dimensional space positioning. In the first step, six transmitters are selected in the code division transmission scheme. This is because there are many transmitters in the whole network, and the time-division scheme for all transmitters will cause a large time overhead and scheduling complexity. Although the positioning accuracy is slightly lower and less stable in the code division transmission scheme, the signal strength can still be indicated by the size of the correlation peak value. Consequently, we can find the six transmitters that are close to the receiver. In the second step, the six selected transmitters transmitt their synchronization sequences in turn at fixed time interval $T$ according to the time division transmission scheme in order to achieve higher and more stable positioning accuracy.
%\subsection{Optimization Objective}
%The objective is to minimize the upper bound given in Eq. \eqref{upbound} subject to the constraint the probability of symbol-level offset is below a low threshold. Note that as $ \alpha $ increases, the probability of $ {\hat t}_{start}=t_{0,0} $ increases, the probability of $ {\hat t}_{start}=t_{0,k} $ decreases and the probability of $ {\hat t}_{start}=t_{2m,k} $ increases. The probability of $ {\hat t}_{start}=t_{2m,k} $ needs to be sufficiently small to avoid significant performance loss of signal detection, which translates to the constraint that $\alpha$ should be lower than a certain threshold. 
%%\begin{align}\label{lowest point}
%%	\exists \alpha_{0}\in \left[0,1\right],~~ s.t.~ \alpha_{0}=\mathop{\arg\min}_{\alpha}\mathrm{E}\left(\bar{e^{2}} \right),
%%\end{align}
%
%In particular, we characterize a more rigorous constraint on the threshold of $ \alpha $ to avoid Case 3. The upper bound on the probability of Case 3 needs to be lower than a certain threshold $\eta$, which should be sufficiently small, such as $ 10^{-8} $, expressed as follows,
%\begin{align}\label{premise}
%	P\left(Case~3 \right) \leq 2 \sum_{m=1}^{\infty} \sum_{k=-n}^{(n-1)} \bar{p}_{2 m, k} \leq \eta.
%\end{align}
%\subsection{Mathematical Expression of the Optimization}
%The optimization of synchronization sequence can be formulated as minimizing the upper bound on MSE under the constraint that the upper bound on the probability of Case 3 needs to be lower than threshold $\eta$. For varying signal intensity $\lambda_{s}$, let $ \Lambda $ denote its definition domain, i.e., $ \lambda_{s} \in \Lambda  $. The mean value of MSE is considered in the domain $\Lambda $, so the optimization can be expressed as follows,
%%	\begin{equation}
%%		\begin{aligned} \label{P}
%%			&\min_{\alpha} \quad \int_{-\frac{T_c}{2}}^{\frac{T_c}{2}}\left(	e_{0,0}^{2} \times \bar{p_{0,0}}+2 \sum_{k=1}^{n-1} e_{0, k}^{2} \times \bar{p_{0, k}}+2 \sum_{m=1}^{\infty} \sum_{k=-(n-1)}^{n} e_{2 m, k}^{2} \times \bar{p_{2 m, k}}\right) p(\varepsilon) d \varepsilon\\
%%			&\begin{array}{r@{\quad}r@{}l@{\quad}l}
%%				s.t. &	2 \sum_{m=1}^{\infty} \sum_{k=-(n-1)}^{n} \bar{p_{2 m, k}} -\eta \leq 0 \\
%%			\end{array}
%%		\end{aligned}
%%	\end{equation}
%%Or form of the optimization problem is like:
%   	\begin{equation}
%   	\begin{aligned} \label{P}
%   		\min_{\alpha } ~~~ & \int_{\lambda_{s} \in \Lambda }  MSE(\alpha| \lambda_{s}) p(\lambda_{s})d\lambda_{s}\\
%   		s.t. ~~~&\int_{\lambda_{s} \in \Lambda }2 \sum_{m=1}^{\infty} \sum_{k=-n}^{(n-1)} \bar{p}_{2 m, k}p(\lambda_{s})d\lambda_{s} \leq \eta, \\
%   		        &0 \leq \alpha \leq 1,
%   	\end{aligned}
%   \end{equation}
%where $ p(\lambda_{s}) $ is the probability density function of $ \lambda_{s} $.
%
%The above optimization problem only involves an one-dimensional parameter $\alpha$, which can be solved via exhaustive search, bisection search, or golden search.





















%\begin{algorithm}[H]
%	\caption{Search Method for the interval $ [0,\alpha_{threshold}] $}
%	\label{alg1}
%	\begin{algorithmic}[1]
%		\Require $ P(Case~3 \textbar \alpha)$, the search accuracy $ h $
%		\Ensure $\alpha_{threshold}$ \\ % 这\\是换行
%		
%		\textbf{Initialize:$ a=0,b=1 $}
%		
%		% while
%		\While{$(b \geq a)$ and $( g \textgreater \eta) $ }\\
%		$ \alpha_{1}=b-h $,$ g =  P(Case~3 \textbar \alpha=\alpha_{1})$
%		\EndWhile 
%		\State $\alpha_{threshold}= \alpha_{1}$.
%		
%	\end{algorithmic}
%\end{algorithm}
%
%We perform Golden Search Method on the interval $ [0,\alpha_{threshold}] $ to find the minimum. 
%\begin{algorithm}[H]
%	\caption{Golden Search Method for the optimization problem \ref{P}}
%	\label{alg2}
%	\begin{algorithmic}[1]
%		\Require $\alpha_{threshold}$, $\mathrm{E}\left(\bar{e^{2}} \right)\left(\alpha\right)$, the search accuracy $ h $
%		\Ensure $\alpha_{0}$ \\ % 这\\是换行
%		
%		\textbf{Initialize:$ a=0,b=\alpha_{threshold} $}\\
%		The insertion point generated by using the golden section method: \\
%		 $ \alpha_{1} = a + 0.382(b-a)$,
%	   	$ \alpha_{2} = a + 0.618(b-a) $
%		% while
%		\While{$\left(b-a \geq h\right)$}
%		\State $f_{1}= \mathrm{E}\left(\bar{e^{2}} \right)\left(\alpha_{1}\right)$,$f_{2}= \mathrm{E}\left(\bar{e^{2}} \right)\left(\alpha_{2}\right)$
%		   \If{$f_{1} \textgreater f_{2}$}
%		          \State  $ a=\alpha_{1},\alpha_{1}=\alpha_{2},\alpha_{2}=a+0.618(b-a) $
%		         
%		          \Else
%		          \State $b=\alpha_{2},\alpha_{2}=\alpha_{1},\alpha_{1}=a+0.382(b-a) $
%		          \EndIf
%		\EndWhile 
%		\State $\alpha_{0}= \frac{\alpha_{1}+\alpha_{2}}{2}$.
%		
%	\end{algorithmic}
%\end{algorithm}


%On the premise \eqref{premise}, the $\alpha$ we picked up should get as close to $\alpha_{0}$ in \ref{lowest point} as it can.
%\subsection{Calculation example}\label{alphaSelect}
%In practice, $ \lambda_{s} $ and $ \lambda_{b} $ are taken from the worst signal-to-noise condition of the current scenario to avoid failed synchronization. The number of chips in one symbol is decided by the clock sampling frequency of the hardware. And extremely small $ p_{2m,k}$ can be ignored when $m \textgreater 10 $.
%
%Set $ \lambda_s = 5 $ and $ \lambda_b = 1 $ as the worst signal-to-noise condition, and the number of chips in one symbol satisfies $ n=100 $.  
%
%We have the optimization result as table \ref{table.alpha}
%\begin{center}
%	\captionof{table}{The optimization of $ \alpha $ for synchronous sequences}
%	\label{table.alpha}
%	\begin{tabular}{| c | c | c | c |}
%		\hline
%		Sequence length $ L $ & $ \alpha_{0}=\mathop{\arg\min}_{\alpha}\mathrm{E}\left(\bar{e^{2}} \right) $ &
%		$ \left\{\alpha \colon 2 \sum_{m=1}^{\infty} \sum_{k=-n}^{n} \bar{p_{2 m, k}} \leq 10^{-8}\right\} $ &
%		final $ alpha_{chosen} $\\ \hline
%		$ 128 $ & $ 0.770 $ &$  \left\{\alpha \colon \alpha \leq 0.719\right\} $ &$ 0.719 $\\ \hline
%		$ 256 $ & $ 0.863 $ &$  \left\{\alpha \colon \alpha \leq 0.853\right\} $ &$ 0.853 $\\ \hline
%		$ 512 $ & $ 0.917 $ &$  \left\{\alpha \colon \alpha \leq 0.913\right\} $ &$ 0.913 $\\ 
%		\hline
%	\end{tabular}
%\end{center}
%
%Then we can get the synchronization sequence which is both reliable and has a high synchronization accuracy with final $ alpha_{chosen} $ corresponding to sequence length. 

%\begin{align}
%	\mathrm{E}\left(\bar{e^{2}} \mid \varepsilon\right)&=E_{1}+E_{2}+E_{3},\\
%	E_{1}&=e_{0,0}^{2} \times \bar{p_{0,0}},\\
%	E_{2}&=2 \sum_{k=1}^{n} e_{0, k}^{2} \times \bar{p_{0, k}},\\
%	E_{3}&=2 \sum_{m=1}^{\infty} \sum_{k=-n}^{n} e_{2 m, k}^{2} \times \bar{p_{2 m, k}},
%\end{align} 
%So as $ \alpha $ increases, $ E_{1}$ increases,$E_{2} $ decreases and $ E_{3} $ increases.


































%\section{Acknowledegments}
%The authors would like to thank Dr. Qian Gao (Futurewei Technology) for his constructive comments and suggestions that improve the quality of this paper.

==> Sec7_Simulation.tex <==
\graphicspath{{figure_yu/FigSim/}}



\section{Verification by Simulation} \label{section.verification by simulating}
%
%Numerical simulations are conducted to verify the derivation in Section \ref{section.Mathematical expectation,variance and covariance of correlation values} and Section \ref{section.estimation of the synchronization accuracy}.

%\subsection{Verification for Statistical Analysis of Correlation Value}\label{veriStat}


==> Sec8_Conclu.tex <==
\section{Conclusion} \label{section.conclusion}
We have designed, prototyped and tested the TDOA positioning system via UV transmission. Based on the synchronization accuracy, the theoretical positioning error is analyzed, which shows satisfactorily agreement with the simulated positioning error. We have also conducted hardware realization as well as three outdoor tests. The average positioning errors obtained from the experiments show agreement with the theoretical results. The positioning error is dominated by the timing synchronization issue of the three transmitters, and can be further reduced via time synchronization among three transmitters.
